Adaptive Econometric Inference under Unknown Dependence: Contrast-Local Validity

Empirical conclusions can depend on how researchers model dependence when constructing standard errors. We develop contrast-local validity, which asks whether a covariance restriction is accurate for the particular coefficient or weighted contrast being reported, even when the restriction is globally misspecified. The method tests target-specific covariance contamination, compares numerically certified structured corrections with an unrestricted benchmark, and adapts inference to the economic target. In a separate growing-block benchmark, valid structure achieves an optimal faster rate for estimating the target variance, while any globally misspecified covariance approximation must fail for some contrast. In a Fama--French calibration where validity is imposed, the feasible selector preserves nominal coverage and reduces variance-estimation root mean squared error by 39 percent. A publicly available FHFA house-price application illustrates target-specific verdicts across regional exposures. Detectability and coverage-risk analyses show when non-rejection is informative and when unrestricted inference should remain primary.

==> Cov_Learn_arxiv_v2/Figures/del/dependence_learning_framework_v4_tikzonly_minimal.tex <==
% TikZ-only file. Include inside a figure environment with:
% \resizebox{\textwidth}{!}{\input{Figures/dependence_learning_framework_v3_tikzonly}}
% Required in main preamble:
% \usepackage{tikz}
% \usetikzlibrary{arrows,positioning,calc}
% This Version 4 preserves Version 3 layout and only increases Part B vertical spacing slightly.

\begin{tikzpicture}[
  >=stealth,
  font=\footnotesize,
  arr/.style={->, line width=0.6pt, black!80},
  panel/.style={draw=black!35, rounded corners=4pt, line width=0.55pt, fill=black!1},
  title/.style={font=\bfseries\footnotesize, text=white, fill=blue!70!black, draw=blue!70!black, rounded corners=3pt, inner xsep=6pt, inner ysep=3pt, align=center},
  flow/.style={draw=blue!65!black, fill=blue!5, rounded corners=3pt, align=center, text width=3.65cm, minimum height=0.72cm, inner sep=3pt},
  profile/.style={draw=green!45!black, fill=green!6, rounded corners=3pt, align=center, text width=3.65cm, minimum height=0.72cm, inner sep=3pt},
  diag/.style={draw=orange!75!black, fill=orange!8, rounded corners=3pt, align=center, text width=2.25cm, minimum height=0.85cm, inner sep=3pt},
  learn/.style={draw=purple!60!black, fill=purple!6, rounded corners=3pt, align=center, text width=2.25cm, minimum height=0.85cm, inner sep=3pt},
  decision/.style={draw=orange!80!black, fill=orange!9, rounded corners=3pt, align=center, text width=3.65cm, minimum height=0.72cm, inner sep=3pt},
  action/.style={draw=red!65!black, fill=red!6, rounded corners=3pt, align=center, text width=3.65cm, minimum height=0.72cm, inner sep=3pt},
  greenbox/.style={draw=green!45!black, fill=green!5, rounded corners=3pt, align=center, text width=2.75cm, minimum height=0.78cm, inner sep=3pt},
  redbox/.style={draw=red!60!black, fill=red!5, rounded corners=3pt, align=center, text width=2.75cm, minimum height=0.78cm, inner sep=3pt}
]

\node[font=\bfseries\normalsize, align=center] at (8.0,0.25)
{Overview of the Dependence Learning Framework};

\node[panel, minimum width=7.25cm, minimum height=10.55cm, anchor=north west] (PA) at (0,-0.15) {};
\node[panel, minimum width=8.35cm, minimum height=10.55cm, anchor=north west] (PB) at (7.50,-0.15) {};
\node[title, minimum width=5.65cm, anchor=north] at (3.625,-0.35) {Part A. Data-to-Decision Pipeline};
\node[title, minimum width=6.50cm, anchor=north] at (11.675,-0.35) {Part B. Identification and Fundamental Limits};

% Part A
\node[flow] (A1) at (3.625,-1.35) {Data\\[-1pt] $\{y_{it},x_{it}\}$};
\node[flow] (A2) at (3.625,-2.55) {Empirical operator\\[-1pt] $\widehat{\Gamma}_n\in\mathcal H$};
\node[flow] (A3) at (3.625,-3.75) {Geometry projection\\[-1pt] $\{\mathcal G_1,\ldots,\mathcal G_K\}$};
\node[profile] (A4) at (3.625,-4.95) {Geometric profile\\[-1pt] $\widehat\omega=(\widehat\omega_1,\ldots,\widehat\omega_K)$};
\node[diag] (A5a) at (1.95,-6.30) {Diagnostics\\[-1pt] $\widehat r_n$};
\node[learn] (A5b) at (5.30,-6.30) {Learning\\[-1pt] $\widehat d$, ambiguity};
\node[decision] (A6) at (3.625,-7.72) {Decision rule\\[-1pt] $a=\delta(\widehat\omega,\widehat r_n)$};
\node[action] (A7) at (3.625,-8.92) {Adaptive inference\\[-1pt] $V_n=V_n(a,\widehat\omega)$};
\draw[arr] (A1) -- (A2); \draw[arr] (A2) -- (A3); \draw[arr] (A3) -- (A4);
\draw[arr] (A4.south west) -- (A5a.north); \draw[arr] (A4.south east) -- (A5b.north);
\draw[arr] (A5a.south) |- (A6.west); \draw[arr] (A5b.south) |- (A6.east); \draw[arr] (A6) -- (A7);

% Part B
\node[font=\bfseries\footnotesize, text=green!40!black, align=center] at (9.65,-1.18)
{Separated geometries\\[-1pt] \normalfont identifiable};
\node[font=\bfseries\footnotesize, text=red!65!black, align=center] at (13.65,-1.18)
{Overlapping geometries\\[-1pt] \normalfont nonidentifiable};
\draw[green!45!black, fill=green!12, line width=0.6pt] (8.65,-1.95) -- (9.25,-1.78) -- (9.72,-2.05) -- (8.98,-2.27) -- cycle;
\draw[blue!65!black, fill=blue!10, line width=0.6pt] (10.20,-2.20) -- (10.90,-2.02) -- (11.18,-1.70) -- (10.38,-1.88) -- cycle;
\draw[<->, >=stealth, black!70, line width=0.5pt] (9.80,-2.05) to[bend left=20] node[above, font=\tiny] {$\theta_{jk}>0$} (10.15,-2.05);
\draw[red!65!black, fill=red!10, line width=0.6pt] (12.20,-1.98) -- (12.98,-1.80) -- (13.25,-2.23) -- (12.42,-2.42) -- cycle;
\draw[blue!65!black, fill=blue!10, line width=0.6pt, opacity=0.75] (12.85,-2.23) -- (13.72,-2.03) -- (14.10,-2.28) -- (13.22,-2.58) -- cycle;
\node[font=\tiny] at (14.08,-2.65) {$\theta_{jk}=0$};

\node[greenbox] (B1) at (9.65,-3.45) {Identification\\[-1pt] \tiny separated tangents};
\node[greenbox] (B2) at (9.65,-4.67) {Consistent profile\\[-1pt] $\widehat\omega\overset{p}{\to}\omega$};
\node[greenbox] (B3) at (9.65,-5.89) {Dependence learning\\[-1pt] $\Pr(\widehat d=d^\star)\to1$};
\node[greenbox] (B4) at (9.65,-7.11) {Oracle inference\\[-1pt] $V_n-V_n^{oracle}=o_p(n^{-1/2})$};
\node[greenbox] (B5) at (9.65,-8.33) {Vanishing regret\\[-1pt] $\mathcal R_n=o(1)$};
\node[redbox] (C1) at (13.65,-3.45) {Fundamental limit\\[-1pt] \tiny overlapping tangents};
\node[redbox] (C2) at (13.65,-4.67) {Indistinguishability\\[-1pt] \tiny no first-order test};
\node[redbox] (C3) at (13.65,-5.89) {Ambiguous profile\\[-1pt] \tiny diffuse $\widehat\omega$};
\node[redbox] (C4) at (13.65,-7.11) {Hybrid action\\[-1pt] \tiny minimax or mixture};
\node[redbox] (C5) at (13.65,-8.33) {Positive regret\\[-1pt] \tiny unavoidable near overlap};
\draw[arr] (B1) -- (B2); \draw[arr] (B2) -- (B3); \draw[arr] (B3) -- (B4); \draw[arr] (B4) -- (B5);
\draw[arr] (C1) -- (C2); \draw[arr] (C2) -- (C3); \draw[arr] (C3) -- (C4); \draw[arr] (C4) -- (C5);

\end{tikzpicture}


==> Cov_Learn_arxiv_v2/Figures/dependence_learning_framework_v4_tikzonly_minimal.tex <==
% TikZ-only file. Include inside a figure environment with:
% \resizebox{\textwidth}{!}{\input{Figures/dependence_learning_framework_v3_tikzonly}}
% Required in main preamble:
% \usepackage{tikz}
% \usetikzlibrary{arrows,positioning,calc}
% This Version 4 preserves Version 3 layout and only increases Part B vertical spacing slightly.

\begin{tikzpicture}[
  >=stealth,
  font=\footnotesize,
  arr/.style={->, line width=0.6pt, black!80},
  panel/.style={draw=black!35, rounded corners=4pt, line width=0.55pt, fill=black!1},
  title/.style={font=\bfseries\footnotesize, text=white, fill=blue!70!black, draw=blue!70!black, rounded corners=3pt, inner xsep=6pt, inner ysep=3pt, align=center},
  flow/.style={draw=blue!65!black, fill=blue!5, rounded corners=3pt, align=center, text width=3.65cm, minimum height=0.72cm, inner sep=3pt},
  profile/.style={draw=green!45!black, fill=green!6, rounded corners=3pt, align=center, text width=3.65cm, minimum height=0.72cm, inner sep=3pt},
  diag/.style={draw=orange!75!black, fill=orange!8, rounded corners=3pt, align=center, text width=2.25cm, minimum height=0.85cm, inner sep=3pt},
  learn/.style={draw=purple!60!black, fill=purple!6, rounded corners=3pt, align=center, text width=2.25cm, minimum height=0.85cm, inner sep=3pt},
  decision/.style={draw=orange!80!black, fill=orange!9, rounded corners=3pt, align=center, text width=3.65cm, minimum height=0.72cm, inner sep=3pt},
  action/.style={draw=red!65!black, fill=red!6, rounded corners=3pt, align=center, text width=3.65cm, minimum height=0.72cm, inner sep=3pt},
  greenbox/.style={draw=green!45!black, fill=green!5, rounded corners=3pt, align=center, text width=2.75cm, minimum height=0.78cm, inner sep=3pt},
  redbox/.style={draw=red!60!black, fill=red!5, rounded corners=3pt, align=center, text width=2.75cm, minimum height=0.78cm, inner sep=3pt}
]

\node[font=\bfseries\normalsize, align=center] at (8.0,0.25)
{Overview of the Dependence Learning Framework};

\node[panel, minimum width=7.25cm, minimum height=10.55cm, anchor=north west] (PA) at (0,-0.15) {};
\node[panel, minimum width=8.35cm, minimum height=10.55cm, anchor=north west] (PB) at (7.50,-0.15) {};
\node[title, minimum width=5.65cm, anchor=north] at (3.625,-0.35) {Part A. Data-to-Decision Pipeline};
\node[title, minimum width=6.50cm, anchor=north] at (11.675,-0.35) {Part B. Identification and Fundamental Limits};

% Part A
\node[flow] (A1) at (3.625,-1.35) {Data\\[-1pt] $\{y_{it},x_{it}\}$};
\node[flow] (A2) at (3.625,-2.55) {Empirical operator\\[-1pt] $\widehat{\Gamma}_T\in\mathcal H$};
\node[flow] (A3) at (3.625,-3.75) {Geometry projection\\[-1pt] $\{\mathcal G_1,\ldots,\mathcal G_K\}$};
\node[profile] (A4) at (3.625,-4.95) {Geometric profile\\[-1pt] $\widehat\omega=(\widehat\omega_1,\ldots,\widehat\omega_K)$};
\node[diag] (A5a) at (1.95,-6.30) {Diagnostics\\[-1pt] $\widehat r_T$};
\node[learn] (A5b) at (5.30,-6.30) {Learning\\[-1pt] $\widehat d$, ambiguity};
\node[decision] (A6) at (3.625,-7.72) {Decision rule\\[-1pt] $a=\delta(\widehat\omega,\widehat r_T)$};
\node[action] (A7) at (3.625,-8.92) {Adaptive inference\\[-1pt] $V_T=V_T(a,\widehat\omega)$};
\draw[arr] (A1) -- (A2); \draw[arr] (A2) -- (A3); \draw[arr] (A3) -- (A4);
\draw[arr] (A4.south west) -- (A5a.north); \draw[arr] (A4.south east) -- (A5b.north);
\draw[arr] (A5a.south) |- (A6.west); \draw[arr] (A5b.south) |- (A6.east); \draw[arr] (A6) -- (A7);

% Part B
\node[font=\bfseries\footnotesize, text=green!40!black, align=center] at (9.65,-1.18)
{Separated geometries\\[-1pt] \normalfont identifiable};
\node[font=\bfseries\footnotesize, text=red!65!black, align=center] at (13.65,-1.18)
{Overlapping geometries\\[-1pt] \normalfont nonidentifiable};
\draw[green!45!black, fill=green!12, line width=0.6pt] (8.65,-1.95) -- (9.25,-1.78) -- (9.72,-2.05) -- (8.98,-2.27) -- cycle;
\draw[blue!65!black, fill=blue!10, line width=0.6pt] (10.20,-2.20) -- (10.90,-2.02) -- (11.18,-1.70) -- (10.38,-1.88) -- cycle;
\draw[<->, >=stealth, black!70, line width=0.5pt] (9.80,-2.05) to[bend left=20] node[above, font=\tiny] {$\theta_{jk}>0$} (10.15,-2.05);
\draw[red!65!black, fill=red!10, line width=0.6pt] (12.20,-1.98) -- (12.98,-1.80) -- (13.25,-2.23) -- (12.42,-2.42) -- cycle;
\draw[blue!65!black, fill=blue!10, line width=0.6pt, opacity=0.75] (12.85,-2.23) -- (13.72,-2.03) -- (14.10,-2.28) -- (13.22,-2.58) -- cycle;
\node[font=\tiny] at (14.08,-2.65) {$\theta_{jk}=0$};

\node[greenbox] (B1) at (9.65,-3.45) {Identification\\[-1pt] \tiny separated tangents};
\node[greenbox] (B2) at (9.65,-4.67) {Consistent profile\\[-1pt] $\widehat\omega\overset{p}{\to}\omega$};
\node[greenbox] (B3) at (9.65,-5.89) {Dependence learning\\[-1pt] $\Pr(\widehat d=d^\star)\to1$};
\node[greenbox] (B4) at (9.65,-7.11) {Oracle inference\\[-1pt] $V_T-V_T^{oracle}=o_p(T^{-1/2})$};
\node[greenbox] (B5) at (9.65,-8.33) {Vanishing regret\\[-1pt] $\mathcal R_T=o(1)$};
\node[redbox] (C1) at (13.65,-3.45) {Fundamental limit\\[-1pt] \tiny overlapping tangents};
\node[redbox] (C2) at (13.65,-4.67) {Indistinguishability\\[-1pt] \tiny no first-order test};
\node[redbox] (C3) at (13.65,-5.89) {Ambiguous profile\\[-1pt] \tiny diffuse $\widehat\omega$};
\node[redbox] (C4) at (13.65,-7.11) {Hybrid action\\[-1pt] \tiny minimax or mixture};
\node[redbox] (C5) at (13.65,-8.33) {Positive regret\\[-1pt] \tiny unavoidable near overlap};
\draw[arr] (B1) -- (B2); \draw[arr] (B2) -- (B3); \draw[arr] (B3) -- (B4); \draw[arr] (B4) -- (B5);
\draw[arr] (C1) -- (C2); \draw[arr] (C2) -- (C3); \draw[arr] (C3) -- (C4); \draw[arr] (C4) -- (C5);

\end{tikzpicture}


==> Cov_Learn_arxiv_v2/results/tables/macros_lambda_bar.tex <==
% Auto-generated by run_simulations.m -- realized factor-loading mean
\newcommand{\lambdaBarRealized}{0.1187}
\newcommand{\lambdaBarZscore}{1.877}


==> Cov_Learn_arxiv_v2/results/tables/table_cigar_profile.tex <==
\begin{tabular}{lc}\toprule
Quantity & Value\\
\midrule
$\omega_C$ (cluster) & 0.161\\
$\omega_F$ (factor) & 0.461\\
$\omega_S$ (sparse) & 0.378\\
$\rho_C$ & 0.812\\
$\rho_F$ & 0.153\\
$\rho_S$ & 0.448\\
$\hat\rho_{\min}$ & 0.153\\
$\hat\Delta_\omega$ & 0.084\\
$\hat\kappa$ & 0.071\\
\bottomrule
\end{tabular}


==> Cov_Learn_arxiv_v2/results/tables/table_cigar_standard_errors.tex <==
\begin{tabular}{lcccccc}\toprule
Coefficient & SE method & $\hat\beta$ & SE & $t$ & $p$ & \\
\midrule
log real price & Homoskedastic & -1.023 & 0.042 & -24.46 & 0.000 & $^{*}$\\
log real price & HC1 & -1.023 & 0.061 & -16.66 & 0.000 & $^{*}$\\
log real price & Cluster-state & -1.023 & 0.224 & -4.57 & 0.000 & $^{*}$\\
log real price & Cluster-year & -1.023 & 0.061 & -16.79 & 0.000 & $^{*}$\\
log real income & Homoskedastic & 0.520 & 0.047 & 11.14 & 0.000 & $^{*}$\\
log real income & HC1 & 0.520 & 0.059 & 8.87 & 0.000 & $^{*}$\\
log real income & Cluster-state & 0.520 & 0.165 & 3.16 & 0.002 & $^{*}$\\
log real income & Cluster-year & 0.520 & 0.082 & 6.34 & 0.000 & $^{*}$\\
log nearby min price & Homoskedastic & -0.117 & 0.054 & -2.17 & 0.030 & $^{*}$\\
log nearby min price & HC1 & -0.117 & 0.063 & -1.85 & 0.064 & \\
log nearby min price & Cluster-state & -0.117 & 0.085 & -1.37 & 0.170 & \\
log nearby min price & Cluster-year & -0.117 & 0.057 & -2.04 & 0.041 & $^{*}$\\
\bottomrule
\end{tabular}


==> Cov_Learn_arxiv_v2/results/tables/table_empirical_inference.tex <==
\begin{tabular}{lccccc}\toprule
Operator & $\widehat\Delta_\omega$ & $\widehat\rho_{\min}$ & $\widehat\kappa$ & Dominant geometry & Profile-guided recommendation\\
\midrule
Covariance & 0.031 & 0.366 & 0.019 & Sparse & Hybrid: report multiple SEs (low $\widehat\kappa$)\\
Correlation & 0.022 & 0.485 & 0.011 & Factor & Hybrid: report multiple SEs (low $\widehat\kappa$)\\
\bottomrule
\end{tabular}


==> Cov_Learn_arxiv_v2/results/tables/table_empirical_profile.tex <==
\begin{tabular}{lcccccccc}\toprule
Operator & $\widehat\omega_C$ & $\widehat\omega_F$ & $\widehat\omega_S$ & $\widehat\rho_C$ & $\widehat\rho_F$ & $\widehat\rho_S$ & $\widehat\rho_{\min}$ & $r$\\
\midrule
Covariance & 0.321 & 0.324 & 0.355 & 0.465 & 0.457 & 0.366 & 0.366 & 1\\
Correlation & 0.293 & 0.364 & 0.342 & 0.619 & 0.485 & 0.529 & 0.485 & 1\\
\bottomrule
\end{tabular}


==> Cov_Learn_arxiv_v2/results/tables/table_empirical_standard_errors.tex <==
\begin{tabular}{lccccc}\toprule
Coefficient & Estimate & White & Sector cluster & Two-way cluster & Common-shock adj.\\
\midrule
Intercept & -0.0005 & 0.0003 & 0.0004 & 0.0006 & 0.0002\\
MKT & 1.0326 & 0.0077 & 0.0432 & 0.0447 & 0.0061\\
SMB & 0.1957 & 0.0125 & 0.0460 & 0.0560 & 0.0097\\
HML & 0.1934 & 0.0121 & 0.0801 & 0.0830 & 0.0095\\
\bottomrule
\end{tabular}


==> Cov_Learn_arxiv_v2/results/tables/table_misspecified_operator.tex <==
\begin{tabular}{lccccc}\toprule
True DGP & Operator Used & $\widehat\omega_C$ & $\widehat\omega_F$ & $\widehat\omega_S$ & $\widehat\rho_{\min}$\\
\midrule
Sparse & Full covariance & 0.282 & 0.318 & 0.401 & 0.844\\
Sparse & Diagonal only & 0.333 & 0.333 & 0.333 & 0.000\\
Cluster & Full covariance & 0.456 & 0.200 & 0.343 & 0.654\\
Cluster & Cluster support removed & 0.309 & 0.376 & 0.315 & 0.715\\
\bottomrule
\end{tabular}


==> Cov_Learn_arxiv_v2/results/tables/table_near_ties.tex <==
\begin{tabular}{lcccc}\toprule
$c$ & $P_B(\widehat d=C)$ & $P_B(\widehat d=F)$ & $P_B(\widehat d=S)$ & $\Delta_\omega$\\
\midrule
-4.0 & 0.000 & 1.000 & 0.000 & 0.673\\
-2.0 & 0.000 & 1.000 & 0.000 & 0.600\\
-1.0 & 0.003 & 0.997 & 0.000 & 0.395\\
0.0 & 0.173 & 0.827 & 0.000 & 0.026\\
1.0 & 0.937 & 0.063 & 0.000 & 0.199\\
2.0 & 1.000 & 0.000 & 0.000 & 0.250\\
4.0 & 1.000 & 0.000 & 0.000 & 0.294\\
\bottomrule
\end{tabular}


==> Cov_Learn_arxiv_v2/results/tables/table_oracle_equivalence.tex <==
\begin{tabular}{lccc}\toprule
DGP & Oracle Coverage & Profile-Guided Coverage & Wrong Procedure\\
\midrule
Cluster & 93.3 & 93.3 & 20.9\\
Factor & 94.2 & 94.2 & 21.8\\
Sparse & 95.8 & 95.8 & 20.6\\
\bottomrule
\end{tabular}


==> Cov_Learn_arxiv_v2/results/tables/table_oracle_tracking.tex <==
\begin{tabular}{lccccccc}\toprule
$\alpha$ & Pop. dominant & $\omega_C-\omega_F$ & $P(\widehat d=d^\star)$ & Cluster SE & Factor SE & $\widehat V^*$ (profile) & $\widehat V_{d^\star}$ (oracle)\\
\midrule
0.000 & Factor & -0.755 & 1.000 & 0.059 & 0.296 & 0.296 & 0.296\\
0.125 & Factor & -0.753 & 1.000 & 0.065 & 0.254 & 0.254 & 0.254\\
0.250 & Factor & -0.749 & 1.000 & 0.057 & 0.178 & 0.178 & 0.178\\
0.375 & Factor & -0.731 & 1.000 & 0.072 & 0.166 & 0.166 & 0.166\\
0.500 & Factor & -0.664 & 1.000 & 0.074 & 0.139 & 0.139 & 0.139\\
0.625 & Factor & -0.392 & 1.000 & 0.062 & 0.089 & 0.089 & 0.089\\
0.750 & Cluster & 0.200 & 0.856 & 0.074 & 0.077 & 0.078 & 0.074\\
0.875 & Cluster & 0.430 & 1.000 & 0.070 & 0.065 & 0.070 & 0.070\\
1.000 & Cluster & 0.464 & 1.000 & 0.075 & 0.068 & 0.075 & 0.075\\
\bottomrule
\end{tabular}


==> Cov_Learn_arxiv_v2/results/tables/table_oracle_tracking_corrected.tex <==
\begin{tabular}{lccccccc}\toprule
$\alpha$ & Pop. dominant & $\omega_C-\omega_F$ & $P(\widehat d=d^\star)$ & Cluster SE & Factor SE (corr.) & $\widehat V^*$ (profile) & $\widehat V_{d^\star}$ (oracle)\\
\midrule
0.000 & Factor & -0.755 & 1.000 & 0.063 & 0.054 & 0.054 & 0.054\\
0.125 & Factor & -0.753 & 1.000 & 0.060 & 0.055 & 0.055 & 0.055\\
0.250 & Factor & -0.749 & 1.000 & 0.069 & 0.061 & 0.061 & 0.061\\
0.375 & Factor & -0.731 & 1.000 & 0.059 & 0.049 & 0.049 & 0.049\\
0.500 & Factor & -0.664 & 1.000 & 0.065 & 0.046 & 0.046 & 0.046\\
0.625 & Factor & -0.392 & 1.000 & 0.076 & 0.053 & 0.053 & 0.053\\
0.750 & Cluster & 0.200 & 0.875 & 0.063 & 0.041 & 0.063 & 0.063\\
0.875 & Cluster & 0.430 & 1.000 & 0.069 & 0.049 & 0.069 & 0.069\\
1.000 & Cluster & 0.464 & 1.000 & 0.061 & 0.053 & 0.061 & 0.061\\
\bottomrule
\end{tabular}


==> Cov_Learn_arxiv_v2/results/tables/table_principal_angles.tex <==
\begin{tabular}{lccc}\toprule
Design & $\theta(T_C^{\mathrm{off}},T_F^{\mathrm{off}})$ & $\theta(T_C^{\mathrm{off}},T_S^{\mathrm{off}})$ & $\theta(T_F^{\mathrm{off}},T_S^{\mathrm{off}})$\\
\midrule
Cluster (pure) & 69.9$^\circ$ & 0.0$^\circ$ & 69.9$^\circ$\\
Factor (pure) & 69.9$^\circ$ & 0.0$^\circ$ & 25.2$^\circ$\\
Sparse (pure) & 69.9$^\circ$ & 0.0$^\circ$ & 67.5$^\circ$\\
Cluster--Sparse & 69.9$^\circ$ & 0.0$^\circ$ & 72.3$^\circ$\\
Factor--Sparse & 69.9$^\circ$ & 0.0$^\circ$ & 25.2$^\circ$\\
\bottomrule
\end{tabular}


==> Cov_Learn_arxiv_v2/results/tables/table_procedure_recommendation.tex <==
\begin{tabular}{lcccccccc}\toprule
DGP & Profile & Mean $\widehat\kappa$ & $P(\widehat d=d^\star)$ & Cluster SE & Factor SE & White SE & $\widehat V^*$ (rec.) & $\widehat V^{\mathrm{avg}}$ (wtd.)\\
\midrule
Cluster & $\widehat\omega_C$ dom. & 0.056 & 1.000 & 0.069 & 0.063 & 0.781 & 0.069 & 0.120\\
Factor & $\widehat\omega_F$ dom. & 0.665 & 1.000 & 0.068 & 0.324 & 0.765 & 0.324 & 0.320\\
\bottomrule
\end{tabular}


==> Cov_Learn_arxiv_v2/results/tables/table_projection_residuals.tex <==
\begin{tabular}{lcccc}\toprule
$\tau$ & $\widehat\rho_C$ & $\widehat\rho_F$ & $\widehat\rho_S$ & $\widehat\rho_{\min}$\\
\midrule
$\tau=0.00$ & 0.954 & 0.266 & 0.870 & 0.266\\
$\tau=0.25$ & 0.952 & 0.289 & 0.868 & 0.289\\
$\tau=0.50$ & 0.951 & 0.309 & 0.866 & 0.309\\
$\tau=1.00$ & 0.948 & 0.352 & 0.863 & 0.352\\
$\tau=2.00$ & 0.942 & 0.434 & 0.859 & 0.434\\
\bottomrule
\end{tabular}


==> Cov_Learn_arxiv_v2/results/tables/table_simulation_designs.tex <==

\begin{tabular}{lll}
\toprule
Design & Dominant Geometry & Purpose \\
\midrule
Cluster & Cluster & Benchmark structured-support dependence \\
Factor & Factor & Benchmark low-rank dependence \\
Sparse & Sparse / none-of-the-above & Network-generated dependence \\
Hybrid & Mixed & Coexistence of multiple geometries \\
Near tie & Ambiguous & Local alternatives and classification uncertainty \\
Oracle sweep & Varies & Profile-guided inference versus oracle benchmark \\
\bottomrule
\end{tabular}


==> Cov_Learn_arxiv_v2/results/tables/table_simulation_profiles.tex <==
\begin{tabular}{lccccccccccccccc}\toprule
Design & $\omega_C$ & $\omega_F$ & $\omega_S$ & $\omega_C^{\mathrm{off}}$ & $\omega_F^{\mathrm{off}}$ & $\omega_S^{\mathrm{off}}$ & $\kappa_0$ & $\widehat\omega_C$ & $\widehat\omega_F$ & $\widehat\omega_S$ & $\widehat\omega_C^{\mathrm{off}}$ & $\widehat\omega_F^{\mathrm{off}}$ & $\widehat\omega_S^{\mathrm{off}}$ & $\mathrm{RMSE}(\widehat{\boldsymbol\omega})$ & $\mathrm{RMSE}(\widehat{\boldsymbol\omega}^{\mathrm{off}})$\\
\midrule
Cluster & 0.567 & 0.103 & 0.330 & 0.689 & 0.028 & 0.284 & 0.405 & 0.456 & 0.201 & 0.343 & 0.497 & 0.170 & 0.334 & 0.150 & 0.245\\
Factor & 0.037 & 0.792 & 0.171 & 0.028 & 0.829 & 0.143 & 0.687 & 0.037 & 0.791 & 0.172 & 0.028 & 0.830 & 0.142 & 0.008 & 0.010\\
Sparse & 0.332 & 0.332 & 0.335 & 0.030 & 0.034 & 0.936 & 0.895 & 0.282 & 0.318 & 0.401 & 0.183 & 0.341 & 0.477 & 0.084 & 0.574\\
Cluster--Factor & 0.067 & 0.753 & 0.180 & 0.053 & 0.802 & 0.145 & 0.547 & 0.067 & 0.748 & 0.185 & 0.053 & 0.798 & 0.149 & 0.022 & 0.019\\
Cluster--Sparse & 0.556 & 0.107 & 0.336 & 0.674 & 0.027 & 0.299 & 0.372 & 0.452 & 0.205 & 0.343 & 0.495 & 0.172 & 0.333 & 0.144 & 0.234\\
Factor--Sparse & 0.037 & 0.792 & 0.171 & 0.028 & 0.829 & 0.143 & 0.685 & 0.038 & 0.790 & 0.173 & 0.028 & 0.829 & 0.143 & 0.009 & 0.011\\
All Three & 0.067 & 0.752 & 0.180 & 0.053 & 0.802 & 0.146 & 0.547 & 0.067 & 0.747 & 0.186 & 0.053 & 0.798 & 0.149 & 0.022 & 0.019\\
Two-way Cluster & 0.664 & 0.165 & 0.171 & 0.797 & 0.106 & 0.097 & 0.692 & 0.529 & 0.254 & 0.217 & 0.611 & 0.250 & 0.139 & 0.170 & 0.242\\
\bottomrule
\end{tabular}


==> Cov_Learn_arxiv_v2/sections/asymptotics.tex <==
\section{Asymptotic Theory}
\label{sec:asymptotics}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

This section establishes consistency and asymptotic normality of the
estimated dependence profile $\widehat\omega$. Asymptotics are
throughout in $T\to\infty$ with $N$ fixed, as stated in
Remark~\ref{rem:asymptotic_regime}.

\begin{assumption}[Asymptotic Linearity of the Dependence Operator]
\label{ass:operatorclt}
There exists a mean-zero random vector $\psi_t\in\mathbb{R}^{N^2}$ such
that
\[
\sqrt T\,
\operatorname{vec}
(
\widehat\Gamma_T-\Gamma_0
)
=
\frac{1}{\sqrt T}
\sum_{t=1}^T
\psi_t
+
o_p(1),
\]
and
\[
\frac{1}{\sqrt T}\sum_{t=1}^T\psi_t
\Rightarrow
N(0,\Omega_\Gamma),
\qquad
\Omega_\Gamma
=
\sum_{h=-\infty}^{\infty}
E(\psi_0\psi_h'),
\]
the series converging absolutely. Because $\{\psi_t\}$ is serially
dependent in general, $\Omega_\Gamma$ is the \emph{long-run} covariance
of $\{\psi_t\}$ and not the contemporaneous second moment
$E(\psi_t\psi_t')$; the distinction matters because $\Xi$ in
Theorem~\ref{thm:profile_clt} is built from $\Omega_\Gamma$.
\end{assumption}

This assumption isolates the sampling uncertainty in the estimated dependence
operator and is the only ingredient needed to transport a time-series central
limit theorem through the geometric projection and normalization maps.

\begin{remark}[Primitive conditions for Assumption~\ref{ass:operatorclt}]
\label{rem:primitive_clt}
Assumption~\ref{ass:operatorclt} is a high-level linear-representation condition
implied by Assumption~\ref{ass:mixing}: the functional CLT for the sample
covariance holds with $\psi_t=\operatorname{vec}(u_tu_t'-\Sigma)$ and
$\Omega_\Gamma$ the long-run variance of $\{u_tu_t'\}$ \citep[Theorem~27.4]{Davidson1994}
when $u_t$ is observed. When $\widehat\Gamma_T$ is built from residuals
$\widehat u_t=u_t-X_t(\widehat\beta-\beta)$, residual replacement is
asymptotically negligible and $\psi_t$ is unchanged: the leading correction
$T^{-1}\sum_t X_t(\widehat\beta-\beta)u_t'$ is a bilinear form in
$\widehat\beta-\beta=O_p(T^{-1/2})$ and the cross-moment
$T^{-1}\sum_t X_t\otimes u_t$, which is itself $O_p(T^{-1/2})$ under the strict
exogeneity $E(X_tu_t')=0$, so the correction is $O_p(T^{-1})=o_p(T^{-1/2})$ and no
first-step term enters $\Omega_\Gamma$. (If strict exogeneity fails, the
cross-moment is $O_p(1)$, the correction is $O_p(T^{-1/2})$, and an explicit
first-step term must be added.) These conditions restrict only the
\emph{temporal} dependence of $\{u_t\}$, not the cross-sectional operator
$\Gamma_0$ (Remark~\ref{rem:two_dependence_notions}).
\end{remark}


\begin{assumption}[Local Projection Regularity]
\label{ass:local_projection_regularity}
For every $d\in\mathfrak D$, the metric projection $P_d$ is single-valued
and locally Lipschitz on a neighborhood of $\Gamma_0$.  For the sparse
geometry, Assumption~\ref{ass:sparse_unique} is a sufficient support-stability
condition once the fixed-support PSD projection is regular.  For the factor
geometry this is a high-level local regularity condition; no global uniqueness
of the nonconvex projection is imposed.
\end{assumption}

Local regularity rules out points at which an arbitrarily small perturbation of
$\Gamma_0$ changes the relevant projection branch or active support; it is a
local learnability requirement, not a global uniqueness claim.

\begin{lemma}[Uniform Consistency of Projection Estimators]
\label{lem:uniform_projection_consistency}
Suppose Assumptions~\ref{ass:local_projection_regularity} and~\ref{ass:mixing} hold. Then
\[
\max_{d\in\mathfrak D}
\|
\widehat P_d-P_{d,0}
\|_F
=
O_p(T^{-1/2}).
\]
\end{lemma}

\begin{theorem}[Consistency of the Dependence Profile]
\label{thm:profile_consistency}
Suppose Assumptions~\ref{ass:local_projection_regularity} and~\ref{ass:mixing} hold. If
$\sum_{d\in\mathfrak D}S_{d,0}>0$, then
$\widehat\omega-\omega_0=O_p(T^{-1/2})$.
\end{theorem}

To state the limiting distribution, define the score map
\[
\mathcal S(\Gamma)
=
\left(
\|P_C(\Gamma)\|_F^2,
\|P_F(\Gamma)\|_F^2,
\|P_S(\Gamma)\|_F^2
\right)'
\]
and let $s_0=\mathcal S(\Gamma_0)=(S_{C,0},S_{F,0},S_{S,0})'$. Let
$\pi(s)=s/(\mathbf 1's)$ denote the normalization map, so that
$\omega_0=\pi(s_0)$.

\begin{assumption}[Projection Differentiability]
\label{ass:projection_differentiability}
Each projection map $P_d$, $d\in\mathfrak D$, is Hadamard differentiable
at $\Gamma_0$, with derivative $\dot P_{d,\Gamma_0}:\mathbb H\to\mathbb H$.
\end{assumption}

Differentiability converts local perturbations of the covariance operator into
local perturbations of the profile, and is precisely the condition that makes
standard errors for profile coordinates and pairwise contrasts available by the
functional delta method.

\begin{remark}[Sufficient conditions]
Assumption~\ref{ass:projection_differentiability} is stronger than
Assumption~\ref{ass:local_projection_regularity}. For a fixed-support cluster or
sparse cone, the projection is continuously differentiable where the active PSD
face is locally stable and the projected point lies on a regular stratum,
reducing to the orthogonal projection onto the support subspace when the PSD
constraint is slack; at an active PSD boundary the derivative is the derivative of
the metric projection onto the active convex cone, not a simple support mask. For
the nonconvex factor geometry, local single-valuedness and Hadamard
differentiability are imposed at a regular projected point (distinct positive
leading eigenvalues help but do not by themselves suffice). The high-level
formulation thus covers all three geometries without asserting invalid global or
boundary formulas.
\end{remark}

\begin{lemma}[Differentiability of the Score Map]
\label{lem:score_differentiability}
Suppose Assumption~\ref{ass:projection_differentiability} holds. Then
the score map $\mathcal S(\cdot)$ is Hadamard differentiable at
$\Gamma_0$, with derivative $\dot{\mathcal S}_{\Gamma_0}$ given
coordinatewise by
\[
\dot S_{d,\Gamma_0}[H]
=
2\,\bigl\langle P_d(\Gamma_0),\,\dot P_{d,\Gamma_0}[H]\bigr\rangle_F,
\qquad d\in\mathfrak D.
\]
\end{lemma}

\begin{theorem}[Asymptotic Distribution of the Dependence Profile]
\label{thm:profile_clt}
Suppose Assumptions~\ref{ass:projection_differentiability} and~\ref{ass:operatorclt} hold. If
$\sum_{d\in\mathfrak D}S_{d,0}>0$, then
\[
\sqrt T
(
\widehat\omega-\omega_0
)
\Rightarrow
N(0,\Xi),
\]
where $\Xi=J_\omega\Omega_\Gamma J_\omega'$, with
$J_\omega=\dot\pi_{s_0}\dot{\mathcal S}_{\Gamma_0}$ and $\dot\pi_{s_0}$
the derivative of $\pi(s)=s/(\mathbf 1's)$ at $s_0$.
\end{theorem}

The theorem makes dependence learning operational: researchers can attach
standard errors to profile coordinates and to the contrasts that determine which
geometry dominates, providing the sampling-uncertainty input for the
classification and near-tie analysis below.

\begin{remark}[Degeneracy of the limiting covariance]
\label{rem:xi_singular}
Because the profile lies on the unit simplex, $\mathbf 1'\widehat\omega=1$
identically, so $\mathbf 1'\Xi\mathbf 1=0$ and $\Xi$ is singular with
rank at most $|\mathfrak D|-1=2$. Inference on $\omega_0$ should
therefore be conducted on any two coordinates (or on contrasts
$\omega_{d}-\omega_{d'}$), using a generalized inverse of $\Xi$ with the
corresponding reduced degrees of freedom; the pairwise contrasts used in
Section~\ref{sec:classification} are of this form and remain
asymptotically $\chi^2$ with the correct degrees of freedom.
\end{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Cov_Learn_arxiv_v2/sections/classification.tex <==
\section{Dependence Diagnostics and Classification}
\label{sec:classification}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The off-diagonal dependence profile is a low-dimensional summary of the
dependence architecture encoded in the empirical operator: large
$\widehat\omega^{\mathrm{off}}_C$, $\widehat\omega^{\mathrm{off}}_F$, and
$\widehat\omega^{\mathrm{off}}_S$ indicate geometric proximity to the cluster,
factor, and sparse classes. It measures relative geometric similarity, not
additive covariance contributions. A natural classification rule uses it
directly,
\begin{equation}
\widehat d
=
\operatorname*{arg\,max}_{d\in\mathfrak D}
\widehat{\omega}^{\mathrm{off}}_d,
\label{eq:classification_rule}
\end{equation}
identifying the class with the largest off-diagonal score. The full dependence
profile is a companion diagnostic and is often more informative than the label
alone: e.g.\ $(0.60,0.30,0.10)$ suggests cluster dominance with meaningful factor
dependence, whereas $(0.35,0.35,0.30)$ suggests hybrid dependence and cautions
against a binary classification.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Statistical Uncertainty for Dependence Scores}
\label{subsec:profile_variance_estimation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Inference for the profile is based on Theorem~\ref{thm:profile_clt},
$\sqrt T(\widehat\omega-\omega_0)\Rightarrow N(0,\Xi)$. With
$e_C,e_F,e_S$ the standard basis, the asymptotic variance of
$\widehat\omega_d$ is $\sigma_d^2=e_d'\Xi e_d$.

\begin{assumption}[Consistent Covariance Estimation]
\label{ass:Xi_estimation}
There exists an estimator \(\widehat{\Xi}\) such that
$\widehat{\Xi}-\Xi=o_p(1)$.
\end{assumption}

Under Assumption~\ref{ass:Xi_estimation}, $\widehat\sigma_d^2=e_d'\widehat\Xi e_d$
consistently estimates $\sigma_d^2$. The construction of $\widehat\Xi$ depends on
the chosen operator: when it admits an asymptotic linear representation, a
plug-in estimator based on the influence function and the delta method may be
used. A universal variance estimator for all possible operators is outside the
paper's scope.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Diagnostic Tests}
\label{subsec:score_diagnostics}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Theorem~\ref{thm:profile_clt} yields standard diagnostics for the profile. The
single-coordinate statistic
$T_d=\sqrt T(\widehat\omega_d-\omega_d^\ast)/\widehat\sigma_d$, with
$\widehat\sigma_d^2=e_d'\widehat\Xi e_d$, is asymptotically $N(0,1)$ under
$H_0:\omega_d=\omega_d^\ast$. More generally, for a full-row-rank $q\times3$
matrix $R_\omega$, the Wald statistic
$W_\omega=T(R_\omega\widehat\omega-r_\omega)'(R_\omega\widehat\Xi
R_\omega')^{-1}(R_\omega\widehat\omega-r_\omega)$ is asymptotically $\chi^2_q$
under $H_0:R_\omega\omega_0=r_\omega$ (using a generalized inverse where
$\Xi$ is singular, per Remark~\ref{rem:xi_singular}). These quantify the
uncertainty in the estimated profile and should be read as diagnostics.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Dominant and Hybrid Dependence}
\label{subsec:dominant_hybrid_classification}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A dominant geometry is suggested when one score substantially exceeds the others
(e.g.\ $\widehat\omega^{\mathrm{off}}_C>\max\{\widehat\omega^{\mathrm{off}}_F,
\widehat\omega^{\mathrm{off}}_S\}$ indicates proximity to the cluster geometry);
hybrid dependence is suggested when several scores are simultaneously large, in
which case the full profile should be reported rather than a single label. This
matters because geometries may overlap---cluster matrices may also be sparse when
cluster sizes are small---so the profile is a continuous description of
dependence architecture rather than a rigid model-selection device.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Dominant Dependence Geometry}
\label{subsec:dominant_geometry}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A central question is whether the estimated profile can identify the dominant
geometry underlying the chosen operator.

\begin{assumption}[Unique Dominant Geometry]
\label{ass:unique_dominant_geometry}

There exists a unique geometry
\(d^{\star}\in\mathfrak D\)
such that

\[
\omega^{\mathrm{off}}_{d^{\star}}
>
\max_{d\neq d^{\star}}
\omega^{\mathrm{off}}_d.
\]
Equivalently, the separation margin
\[
\Delta_{\omega^{\mathrm{off}}}
=
\omega^{\mathrm{off}}_{d^{\star}}
-
\max_{d\neq d^{\star}}
\omega^{\mathrm{off}}_d
\]
satisfies $
\Delta_{\omega^{\mathrm{off}}}>0$.

\end{assumption}

Under Assumption~\ref{ass:unique_dominant_geometry}, define
\begin{equation}
d^{\star}
=
\argmax_{d\in\mathfrak D}
\omega_d^{\mathrm{off}},
\label{eq:dominant_geometry}
\end{equation}
the population dominant geometry. The assumption rules out knife-edge cases in
which two or more geometries have exactly the same population score, a separation
condition common in model selection and classification. Throughout, $P_{\Gamma_0}$
denotes probability under the sample law $P_{\Gamma_0}^T$ of
Assumption~\ref{ass:lan}, under which all stochastic-order statements and
probabilities involving $\widehat\omega$ and $\widehat d$ are taken.

\begin{proposition}[Classification Error Bound]
\label{prop:classification_bound}

Suppose Assumption
\ref{ass:unique_dominant_geometry}
holds. Then
\[
P_{\Gamma_0}(\widehat d\neq d^\star)
\leq
P_{\Gamma_0}
\left(
\max_{d\in\mathfrak D}
|
\widehat\omega_d^{\mathrm{off}}-\omega_d^{\mathrm{off}}
|
\ge
\frac{\Delta_{\omega^{\mathrm{off}}}}{2}
\right),
\]
where
\[
\Delta_{\omega^{\mathrm{off}}}
=
\omega_{d^\star}^{\mathrm{off}}
-
\max_{d\neq d^\star}
\omega_d^{\mathrm{off}}.
\]
\end{proposition}

Classification error can occur only when profile-estimation error exceeds one
half of the population separation margin, linking the finite-sample reliability
of the discrete recommendation to a continuous, estimable geometric quantity.

\begin{theorem}[Consistency of Dominant-Geometry Classification]
\label{thm:dominant_geometry_consistency}

Suppose the consistency conditions of
Proposition~\ref{prop:joint_profile_consistency} hold, including
positivity of the off-diagonal normalizing denominator, and
Assumption~\ref{ass:unique_dominant_geometry} holds. Then

\[
P\!\left(
\widehat d=d^{\star}
\right)
\longrightarrow
1.
\]

\end{theorem}

Theorem~\ref{thm:dominant_geometry_consistency} shows that the
\emph{off-diagonal} dependence profile consistently identifies the dominant
covariance geometry whenever the dominant off-diagonal similarity score is
separated from the remaining scores. Consequently, the off-diagonal dependence
profile is not merely a descriptive summary of dependence but also provides a
statistically consistent basis for dependence classification.

\begin{remark}[Relation to Statistical Classification]

Theorem~\ref{thm:dominant_geometry_consistency}
is analogous to consistency results in model selection and statistical
classification. The distinguishing feature here is that the objects
being classified are covariance geometries rather than parametric
models.

\end{remark}

The classification result provides a formal justification for using the
estimated off-diagonal dependence profile as a guide for procedure recommendation. The implications for inference are developed formally in Section \ref{sec:profile_guided_inference}.
\begin{theorem}[Local Alternatives and Near-Ties]
\label{thm:local_ties}

Suppose

\[
\sqrt T
\left(
\widehat\omega^{\mathrm{off}}-\omega_T^{\mathrm{off}}
\right)
\Rightarrow
N(0,\Xi_{\mathrm{off}}),
\]
where
\[
\omega_T^{\mathrm{off}}
=
(\omega_{C,T}^{\mathrm{off}},\omega_{F,T}^{\mathrm{off}},\omega_{S,T}^{\mathrm{off}})'.
\]

Assume that two geometries,
\(d_1\) and \(d_2\),
satisfy

\[
\omega_{d_1,T}^{\mathrm{off}}
-
\omega_{d_2,T}^{\mathrm{off}}
=
\frac{c}{\sqrt T},
\]
for some constant \(c\in\mathbb R\), while all remaining scores remain
separated by positive constants. Assume the contrast direction
$e=e_{d_1}-e_{d_2}$ satisfies $e'\Xi_{\mathrm{off}} e>0$, so that the pairwise contrast
is asymptotically nondegenerate. Let $P_{\Gamma_T}$ denote probability under the triangular sequence
whose population profile is $\omega_T^{\mathrm{off}}$. Then
\[
P_{\Gamma_T}(\widehat d=d_1)
\]
converges to a nondegenerate limit lying strictly between zero and one,
equal to $\Phi\!\bigl(c/\sqrt{e'\Xi_{\mathrm{off}}e}\bigr)$.

\end{theorem}

A local near-tie is not a defect of the method but a region in which the data
contain only limited first-order evidence favoring one geometry; the
nondegenerate selection probability records that uncertainty rather than
producing an artificially decisive recommendation.
\begin{remark}[Near-Ties]
\label{rem:near_ties}

When the separation margin
\(\Delta_{\omega^{\mathrm{off}}}\)
is close to zero, small sampling fluctuations may alter the dominant
geometry classification. In such situations, the off-diagonal dependence
profile $
\widehat{\omega}^{\mathrm{off}}
=
(\widehat{\omega}_C^{\mathrm{off}},
  \widehat{\omega}_F^{\mathrm{off}},
  \widehat{\omega}_S^{\mathrm{off}})'
$ is typically more informative than the discrete classifier
\(\widehat d\).  In this regime the recommended output is therefore the
profile, its contrast uncertainty, and multiple or hybrid inferential actions,
rather than a single geometry label.
\end{remark}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Cov_Learn_arxiv_v2/sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
This paper studies a prior problem usually resolved before formal inference
begins: which dependence structure should guide the inferential procedure?
Rather than treating that structure as known, we represent candidate mechanisms
as covariance geometries, estimate their relative empirical support through
projection, and use the resulting profile to guide procedure choice. The central
contribution is not another covariance estimator or robust variance formula but a
unified framework for learning dependence that is relevant for inference.

The framework connects four steps usually treated separately: an estimable
dependence operator is projected onto a dictionary of covariance geometries; the
full and off-diagonal profiles summarize overall covariance fit and
cross-sectional dependence; local projection regularity and geometric separation
determine whether a dominant geometry can be learned, while tangent-space overlap
characterizes first-order ambiguity; and a decision rule maps the off-diagonal
profile into an inference procedure. Under a uniquely separated dominant geometry
and the profile--loss compatibility condition, this rule is asymptotically
equivalent to an infeasible oracle and has vanishing regret. The profile is a
low-dimensional diagnostic relative to a chosen dictionary, not a structural
identification device: a dominant component indicates which geometry receives the
strongest support for inference, a near tie signals intrinsic ambiguity when
tangent directions overlap, and a large minimum residual signals that the
dictionary itself is inadequate. The framework thus produces not only a
recommendation but also diagnostics governing how much confidence to place in it.

The broader implication is a change in the order of econometric reasoning:
instead of asking only which robust covariance estimator to use, the researcher
first asks what dependence structure the operator supports, how sharply it is
separated from alternatives, and what that implies for inference---covariance
geometry supplying the representation, the profile the diagnostic, geometric
separation the learnability criterion, and decision theory the inferential
action. The analysis deliberately fixes the cross-sectional dimension and a finite
dictionary, isolating the learning and decision problems; important extensions
include joint $(N,T)$ asymptotics, expanding or data-driven dictionaries, spatial
and network geometries, nonlinear operators, and decision rules that combine
rather than select procedures near ties.

{\small
\begin{center}
\begin{tabular}{p{0.24\textwidth}p{0.66\textwidth}}
\toprule
Diagnostic pattern & Recommended reporting strategy \\
\midrule
Large margin, small minimum residual & Report the matched procedure as the
primary specification and document the profile diagnostics. \\
Small margin, adequate dictionary fit & Treat the result as genuine ambiguity;
report multiple geometry-specific procedures or a pre-specified hybrid rule. \\
Large minimum residual & Regard the candidate dictionary as inadequate and
avoid a geometry-specific recommendation without expanding the dictionary. \\
Full/off-diagonal profiles disagree & Explain whether diagonal heterogeneity or
cross-sectional dependence drives the difference and base procedure choice on
the off-diagonal profile. \\
\bottomrule
\end{tabular}
\end{center}
}

\subsection*{Practical Guidance for Applied Researchers} On constructing the dictionary: include a cluster geometry when units plausibly share group-level shocks (industry, region, cohort); a factor geometry when a few pervasive drivers move most units together; and a sparse geometry when dependence is localized or network-based. When in doubt, include a candidate and let the profile and residual adjudicate---an over-inclusive dictionary costs precision, not validity. On using the output: match the operator to the inferential target; treat a nearly uniform profile with small $\widehat\kappa$ as genuine ambiguity and report several procedures; prefer the hybrid rule when $\widehat\Delta_{\omega^{\mathrm{off}}}$ is within sampling error of zero; read a large $\widehat\rho_{\min}$ as dictionary inadequacy; and when one geometry clearly dominates with small residual, the matched procedure inherits the oracle guarantees of Section~\ref{sec:profile_guided_inference}. The profile is invariant to positive rescalings of the operator but not to its definition, which should be reported; the projection residuals quantify the information the summary discards, and dictionary adequacy is testable through $\widehat\rho_{\min}$.


==> Cov_Learn_arxiv_v2/sections/dependence_learning_conceptual_figure_tikz.tex <==
% Requires in the preamble:
% \usepackage{tikz}
% \usetikzlibrary{arrows.meta,calc}
% \usepackage{graphicx}
% \usepackage{amsmath,amssymb}

\begin{figure}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tikzpicture}[
    >=Latex,
    font=\footnotesize,
    line/.style={-{Latex[length=2.2mm,width=1.3mm]}, line width=0.5pt},
    panel/.style={rectangle, rounded corners=5pt, draw=blue!65, fill=white, line width=0.8pt},
    titlebar/.style={rectangle, rounded corners=3pt, draw=blue!70!black, fill=blue!70!black,
        text=white, font=\bfseries\footnotesize, align=center, inner ysep=3pt},
    stepblue/.style={rectangle, rounded corners=3pt, draw=blue!60, fill=blue!4,
        align=center, text width=7.2cm, minimum height=0.90cm, inner xsep=5pt, inner ysep=4pt, line width=0.45pt},
    stepgreen/.style={rectangle, rounded corners=3pt, draw=green!45!black, fill=green!5,
        align=center, text width=7.35cm, minimum height=1.00cm, inner xsep=5pt, inner ysep=4pt, line width=0.45pt},
    sideorange/.style={rectangle, rounded corners=3pt, draw=orange!80!black, fill=orange!7,
        align=left, text width=4.35cm, minimum height=2.65cm, inner xsep=6pt, inner ysep=6pt, line width=0.45pt},
    sidepurple/.style={rectangle, rounded corners=3pt, draw=purple!70, fill=purple!6,
        align=left, text width=4.55cm, minimum height=2.65cm, inner xsep=6pt, inner ysep=6pt, line width=0.45pt},
    steporange/.style={rectangle, rounded corners=3pt, draw=orange!80!black, fill=orange!7,
        align=center, text width=7.35cm, minimum height=1.00cm, inner xsep=5pt, inner ysep=4pt, line width=0.45pt},
    stepred/.style={rectangle, rounded corners=3pt, draw=red!60, fill=red!5,
        align=center, text width=7.35cm, minimum height=1.15cm, inner xsep=5pt, inner ysep=4pt, line width=0.45pt},
    theorygreen/.style={rectangle, rounded corners=3pt, draw=green!45!black, fill=green!5,
        align=center, text width=4.15cm, minimum height=1.15cm, inner xsep=4pt, inner ysep=4pt, line width=0.45pt},
    theoryred/.style={rectangle, rounded corners=3pt, draw=red!55, fill=red!5,
        align=center, text width=4.15cm, minimum height=1.15cm, inner xsep=4pt, inner ysep=4pt, line width=0.45pt}
]

% =====================================================
% Part A: data-to-decision pipeline
% =====================================================
\node[panel, minimum width=10.7cm, minimum height=16.1cm, anchor=north west] (panelA) at (0,0) {};
\node[titlebar, minimum width=8.1cm, anchor=north] at ([yshift=-0.18cm]panelA.north)
{Part A. The Data-to-Decision Pipeline};
\node[font=\itshape, align=center, text width=9.8cm, anchor=north] at ([yshift=-0.90cm]panelA.north)
{From observed data to adaptive inference via dependence learning.};

\node[stepblue, anchor=north] (A1) at ([yshift=-1.80cm]panelA.north)
{\textbf{1. Observed data}\\[-1pt]$\{y_{it},x_{it}\}$};
\node[stepblue, anchor=north] (A2) at ([yshift=-3.15cm]panelA.north)
{\textbf{2. Estimate dependence operator}\\[-1pt]$\widehat{\Gamma}_T\in\mathcal H$};
\node[stepblue, anchor=north] (A3) at ([yshift=-4.50cm]panelA.north)
{\textbf{3. Project onto covariance geometries}\\[-1pt]$\{\mathcal G_1,\ldots,\mathcal G_K\}$};
\node[stepgreen, anchor=north] (A4) at ([yshift=-5.85cm]panelA.north)
{\textbf{4. Geometric dependence profile}\\[-1pt]$\omega=(\omega_1,\ldots,\omega_K)\in\Delta^{K-1}$};
\node[stepgreen, anchor=north] (A5) at ([yshift=-7.35cm]panelA.north)
{\textbf{5. Estimated profile}\\[-1pt]$\widehat{\omega}=(\widehat{\omega}_1,\ldots,\widehat{\omega}_K)$};

\node[sideorange, anchor=north west] (A6a) at ([xshift=0.45cm,yshift=-8.95cm]panelA.north west)
{\centering\textbf{6a. Projection diagnostics}\par\vspace{3pt}
$\bullet$ Dictionary projection residual $\widehat r_T$\\[3pt]
$\bullet$ Misspecification assessment\\[3pt]
$\bullet$ Absolute fit of the dictionary};

\node[sidepurple, anchor=north east] (A6b) at ([xshift=-0.45cm,yshift=-8.95cm]panelA.north east)
{\centering\textbf{6b. Dependence learning}\par\vspace{3pt}
$\bullet$ Identify dominant geometry\\[-1pt]
\hspace*{0.4cm}$\widehat d=\arg\max_k\widehat\omega_k$\\[3pt]
$\bullet$ Assess ambiguity\\[3pt]
$\bullet$ Quantify uncertainty};

\node[steporange, anchor=north] (A7) at ([yshift=-12.35cm]panelA.north)
{\textbf{7. Decision rule}\\[-1pt]
$\delta(\widehat\omega,\widehat r_T)\mapsto a\in\mathcal A$};
\node[stepred, anchor=north] (A8) at ([yshift=-13.90cm]panelA.north)
{\textbf{8. Adaptive inference action}\\[-1pt]
Implement dependence-robust procedure\\[-1pt]
$V_T=V_T(a,\widehat\omega)$};

\draw[line] (A1) -- (A2);
\draw[line] (A2) -- (A3);
\draw[line] (A3) -- (A4);
\draw[line] (A4) -- (A5);
\draw[line] (A5.south) -- ++(0,-0.36) -| (A6a.north);
\draw[line] (A5.south) -- ++(0,-0.36) -| (A6b.north);
\draw[line] (A6a.south) |- (A7.west);
\draw[line] (A6b.south) |- (A7.east);
\draw[line] (A7) -- (A8);

% =====================================================
% Part B: geometric regimes and consequences
% =====================================================
\node[panel, minimum width=10.0cm, minimum height=16.1cm, anchor=north west] (panelB) at (11.05,0) {};
\node[titlebar, minimum width=8.7cm, anchor=north] at ([yshift=-0.18cm]panelB.north)
{Part B. Geometric Regimes and Inferential Consequences};
\node[font=\itshape, align=center, text width=8.9cm, anchor=north] at ([yshift=-0.90cm]panelB.north)
{Theoretical dichotomy determined by the geometry of covariance classes.};

\node[draw=green!45!black, fill=green!3, rounded corners=4pt,
      minimum width=4.55cm, minimum height=13.95cm, anchor=north west, line width=0.55pt]
      (Bleftpanel) at ([xshift=0.45cm,yshift=-1.78cm]panelB.north west) {};
\node[draw=red!55, fill=red!3, rounded corners=4pt,
      minimum width=4.55cm, minimum height=13.95cm, anchor=north east, line width=0.55pt]
      (Brightpanel) at ([xshift=-0.45cm,yshift=-1.78cm]panelB.north east) {};

\node[font=\bfseries\color{green!40!black}, align=center, text width=4.2cm, anchor=north]
      (Bltitle) at ([yshift=-2.08cm]panelB.north west -| Bleftpanel.center)
{Separated geometries\\(identifiable regime)};
\node[font=\bfseries\color{red!60!black}, align=center, text width=4.2cm, anchor=north]
      (Brtitle) at ([yshift=-2.08cm]panelB.north east -| Brightpanel.center)
{Overlapping geometries\\(nonidentifiable regime)};

\node[theorygreen, anchor=north] (B1) at ([yshift=-3.65cm]panelB.north west -| Bleftpanel.center)
{\textbf{Identification}\\[-1pt]$\theta_{jk}>0$};
\node[theorygreen, anchor=north] (B2) at ([yshift=-5.90cm]panelB.north west -| Bleftpanel.center)
{\textbf{Consistent profile}\\[-1pt]$\widehat\omega\overset{p}{\longrightarrow}\omega$};
\node[theorygreen, anchor=north] (B3) at ([yshift=-8.15cm]panelB.north west -| Bleftpanel.center)
{\textbf{Dependence learning}\\[-1pt]$P_{\Gamma_0}(\widehat d=d^\star)\to1$};
\node[theorygreen, anchor=north] (B4) at ([yshift=-10.40cm]panelB.north west -| Bleftpanel.center)
{\textbf{Oracle adaptivity}\\[-1pt]$\sqrt T\{V_T-V_T^{\mathrm{oracle}}\}=o_p(1)$};
\node[theorygreen, anchor=north] (B5) at ([yshift=-12.65cm]panelB.north west -| Bleftpanel.center)
{\textbf{Vanishing regret}\\[-1pt]$\mathcal R_n=o(1)$};

\draw[line] (B1) -- (B2);
\draw[line] (B2) -- (B3);
\draw[line] (B3) -- (B4);
\draw[line] (B4) -- (B5);

\node[theoryred, anchor=north] (C1) at ([yshift=-3.65cm]panelB.north east -| Brightpanel.center)
{\textbf{Fundamental limit}\\[-1pt]$\theta_{jk}=0$};
\node[theoryred, anchor=north] (C2) at ([yshift=-5.90cm]panelB.north east -| Brightpanel.center)
{\textbf{Local indistinguishability}\\[-1pt]No first-order test};
\node[theoryred, anchor=north] (C3) at ([yshift=-8.15cm]panelB.north east -| Brightpanel.center)
{\textbf{Ambiguous profile}\\[-1pt]$\widehat\omega$ remains diffuse};
\node[theoryred, anchor=north] (C4) at ([yshift=-10.40cm]panelB.north east -| Brightpanel.center)
{\textbf{Hybrid / robust action}\\[-1pt]Mixture or minimax rule};
\node[theoryred, anchor=north] (C5) at ([yshift=-12.65cm]panelB.north east -| Brightpanel.center)
{\textbf{Positive regret unavoidable}\\[-1pt]No uniformly oracle rule};

\draw[line] (C1) -- (C2);
\draw[line] (C2) -- (C3);
\draw[line] (C3) -- (C4);
\draw[line] (C4) -- (C5);

% Bottom note
\node[draw=blue!55, dashed, rounded corners=3pt, align=center, text width=19.4cm,
      fill=blue!2, inner xsep=5pt, inner ysep=6pt, anchor=north]
      at (10.55,-16.55)
{Part A summarizes the data-to-decision pipeline: estimate a dependence operator, construct the geometric dependence profile $\widehat\omega$, conduct diagnostics and learning, and select an inference action. Part B summarizes the two geometric regimes that determine the possibilities and limits of dependence learning and adaptive inference.};

\end{tikzpicture}%
}
\caption{From dependence learning to adaptive inference. Part A summarizes the data-to-decision pipeline: observed data are used to estimate a dependence operator, which is projected onto candidate covariance geometries to construct the full and off-diagonal dependence profiles $(\widehat\omega,\widehat\omega^{\mathrm{off}})$. The off-diagonal profile is primary for classification, while the full profile and projection diagnostics are then mapped into an inference action through a decision rule. Part B summarizes the two geometric regimes underlying the theory. When covariance geometries are separated, the dependence profile is identifiable, dependence learning is consistent, and profile-guided inference achieves oracle equivalence with vanishing regret. When covariance geometries overlap, local indistinguishability generates intrinsic ambiguity and motivates hybrid or robust inference actions.}
\label{fig:dependence-learning-framework}
\end{figure}


==> Cov_Learn_arxiv_v2/sections/empirical.tex <==
\section{Empirical Illustration}
\label{sec:empirical}
Throughout, we report the full profile $\widehat\omega$ and its off-diagonal
companion $\widehat\omega^{\mathrm{off}}$; the latter is the primary
classification and procedure-selection estimand, the former records overall
covariance fit. We present two complementary applications. The first, using
Fama--French industry portfolios, is a transparent case in which the dictionary
fits only weakly, so the diagnostics correctly report \emph{ambiguity}. The
second, using the Baltagi cigarette-demand panel, is \emph{consequential}: the
significance of an economically important coefficient depends on which
cross-sectional dependence structure is assumed for the standard errors, and the
profile identifies which structure the data exhibit. Together they show the
diagnostics behaving honestly when the dictionary fits poorly and decisively when
it fits well.

We use the Fama--French 49 industry portfolios and three factors from the data
library of \citet{FamaFrench1993} and \citet{FamaFrenchDataLibrary}. Industry
portfolio returns are well suited to the framework: they may exhibit cluster
dependence (industries group into sectors), factor dependence (returns load on
common market-wide shocks), and sparse dependence (some industries are linked
through input--output relations or supply chains more than others).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Data and Regression Specification}
\label{subsec:empirical_data}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The analysis uses monthly excess returns on the 49 industry portfolios and the
market, SMB, and HML factors from the Kenneth R. French Data Library
\citep{FamaFrenchDataLibrary}. Let $R_{it}$ be the excess return on portfolio
$i$ in month $t$ ($i=1,\ldots,N$, $t=1,\ldots,T$, $N=49$). Ken French's raw files
code an industry-month as missing (via a numerical sentinel) whenever too few
firms are available; we drop every month in which any of the 49 industries is
flagged missing, restricting the sample to $T=682$ months (July 1969--April
2026). We estimate the factor model
\begin{equation}
R_{it}
=
\alpha_i
+
\beta_{iM} MKT_t
+
\beta_{iS} SMB_t
+
\beta_{iH} HML_t
+
u_{it},
\label{eq:empirical_factor_model}
\end{equation}
stack the residuals as $\widehat u_t=(\widehat u_{1t},\ldots,\widehat u_{Nt})'$,
and form the baseline residual covariance operator
\begin{equation}
\widehat\Gamma
=
\frac{1}{T}
\sum_{t=1}^{T}
\widehat u_t\widehat u_t'
\label{eq:empirical_operator}
\end{equation}
together with the residual correlation operator
$\widehat\Gamma^{COR}=\widehat D^{-1/2}\widehat\Gamma\widehat D^{-1/2}$,
$\widehat D=\operatorname{diag}(\widehat\Gamma)$. The covariance operator
preserves cross-industry volatility differences; the correlation operator focuses
on dependence geometry after normalizing scale.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Dependence Classes and Projections}
\label{subsec:empirical_classes}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We project the empirical operator onto the cluster, factor, and sparse
geometries; the algorithms are those of Online Appendix~B. For the
\textbf{cluster} geometry we use a one-way specification based on the
Fama--French 10-sector classification, with membership $g(i)\in\{1,\ldots,G\}$
and support $(M_C)_{ij}=\ind\{g(i)=g(j)\}$. Because this is a one-way partition
and $\widehat\Gamma$ is PSD, the exact projection is the block mask
$\widehat P_C=M_C\odot\widehat\Gamma$ (each retained principal block is PSD; for
overlapping multiway supports the code instead solves the PSD-constrained
fixed-support projection). The \textbf{factor} projection
$\widehat P_F=L^*+D^*$ ($L^*$ rank-$r$ PSD, $D^*$ diagonal) is computed by the
alternating algorithm of Online Appendix~B, with $r$ selected by an
eigenvalue-ratio criterion on $\widehat\Gamma-\widehat D$ (robustness:
$r\in\{1,2,3\}$). The \textbf{sparse} projection jointly selects an off-diagonal
support of size at most $k_S$ and solves a PSD-constrained least-squares problem
on it; since exhaustive search is combinatorial, the code retains the $k_S$
largest off-diagonal entries of $\widehat\Gamma$ and projects onto the PSD cone
on that fixed support via Dykstra's algorithm---a feasible approximation to the
population metric projection, not a claim that hard thresholding alone solves the
global nonconvex problem.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Estimated Dependence Profiles and Residual Diagnostics}
\label{subsec:empirical_profile}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We apply the estimated profile and projection-residual diagnostics of
Sections~\ref{subsec:similarity_score_estimation}
and~\ref{subsec:projection_residuals} to $\widehat\Gamma$. The profile describes
which geometry provides the strongest \emph{relative} fit; the residuals assess
\emph{absolute} fit, with a large $\widehat\rho_{\min}$ signaling that no
candidate geometry approximates the operator closely even if one receives the
largest relative score. In this application a large $\widehat\omega_C$ reflects
dependence concentrated within broad industry sectors, a large
$\widehat\omega_F$ low-rank common components not absorbed by the observed
factors, and a large $\widehat\omega_S$ dependence concentrated among a small
subset of industry pairs.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Empirical Results}
\label{subsec:empirical_results}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Table~\ref{tab:empirical_profile} reports the estimated dependence
profiles and projection-residual diagnostics for the residual covariance
and correlation operators.

\begin{table}[!ht]
\centering
\caption{Dependence Profiles and Projection-Residual Diagnostics for Industry Portfolio Residuals}
\label{tab:empirical_profile}
\inputIfExists{results/tables/table_empirical_profile.tex}
\begin{minipage}{0.92\textwidth}
\footnotesize
\emph{Notes:}
\vspace{0.4em}
The table reports estimated similarity scores
\((\widehat\omega_C,\widehat\omega_F,\widehat\omega_S)\)
and projection-residual diagnostics
\((\widehat\rho_C,\widehat\rho_F,\widehat\rho_S,\widehat\rho_{\min})\)
using residuals from the industry-level Fama--French regression in
\eqref{eq:empirical_factor_model}. The covariance operator preserves
scale differences across industries, while the correlation operator
normalizes industry-specific residual volatility. The similarity scores
are relative geometric proximity measures and should not be interpreted
as additive variance shares. The residual diagnostics measure absolute
distance from the empirical operator to each covariance geometry.
\end{minipage}
\end{table}

Table~\ref{tab:empirical_profile} reveals a hybrid dependence structure
in which no single covariance geometry dominates and none provides a
close absolute fit.

\textit{Covariance and correlation operators.}
The three similarity scores are close, $\widehat\omega_C=0.321$,
$\widehat\omega_F=0.324$, $\widehat\omega_S=0.355$, with the sparse score
marginally largest and a substantial minimum residual $\widehat\rho_{\min}=0.366$
(attained by the sparse projection). Residual co-movement among the 49
industries---after removing the three Fama--French factors---is thus not well
summarized by any single geometry: sector clustering, common factor structure,
and localized sparse dependence all receive comparable, individually limited
support, and the large $\widehat\rho_{\min}$ signals that the dictionary itself
is, in absolute terms, incomplete for this dataset. Normalizing by industry
volatility shifts the off-diagonal profile mildly toward factor dominance
($\widehat\omega_F^{\mathrm{off}}=0.364$, with sparse $0.342$ and cluster $0.293$
close behind) and raises the minimum residual to $\widehat\rho_{\min}=0.485$.

\textit{Standard errors and recommendation.}
Sector-clustered and two-way clustered standard errors are roughly
$5.6$--$5.8\times$ the White standard error for the market factor
($0.043$--$0.045$ vs.\ $0.008$), while the common-shock adjustment is smaller
($0.006$); the wide spread across procedures (reported in full in Online
Appendix~F) is itself a symptom of the hybrid structure.
Table~\ref{tab:empirical_inference} reports the confidence index and
recommendation for each operator.

\begin{table}[!ht]
\centering
\caption{Profile-Guided Inference Recommendation for Industry Portfolio Residuals}
\label{tab:empirical_inference}
\resizebox{\textwidth}{!}{%
\inputIfExists{results/tables/table_empirical_inference.tex}
}
\begin{minipage}{0.99\textwidth}
\footnotesize
\vspace{0.4em}
\emph{Notes:}
The table reports the separation margin
$\widehat\Delta_{\omega^{\mathrm{off}}}=\max_d\widehat\omega_d^{\mathrm{off}}-\max_{d\neq\widehat d}\widehat\omega_d^{\mathrm{off}}$,
the minimum projection residual $\widehat\rho_{\min}$, the procedure
confidence index $\widehat\kappa=(1-\widehat\rho_{\min})\widehat\Delta_{\omega^{\mathrm{off}}}$,
the estimated dominant geometry, and the implied profile-guided
recommendation. A small $\widehat\kappa$ indicates either near-tie
separation or poor dictionary fit; the recommended response is to report
inference from multiple procedures.
\end{minipage}
\end{table}

Both operators yield small confidence indices: $\widehat\kappa=0.019$ for the
covariance operator ($\widehat\Delta_{\omega^{\mathrm{off}}}=0.031$,
$\widehat\rho_{\min}=0.366$) and $\widehat\kappa=0.011$ for the correlation
operator ($\widehat\Delta_{\omega^{\mathrm{off}}}=0.022$,
$\widehat\rho_{\min}=0.485$). These low values correctly indicate a genuinely
hybrid structure that the dictionary describes only partially, so no single
procedure can be recommended with high confidence, and the framework prescribes
reporting several procedures and documenting sensitivity---exactly the spread
documented in Online Appendix~F.

This example illustrates a key advantage of the proposed framework
over a priori procedure selection.
A researcher who assumes cluster dependence and uses sector-clustered
standard errors is implicitly claiming $\widehat\kappa\approx 1$ for
the cluster geometry---a claim the data refute, since the cluster score
is not even the largest of the three under either operator.
A researcher who learns the profile first discovers the hybrid
structure, obtains $\widehat\kappa$ close to zero, and is correctly
directed to report multiple procedures rather than to commit to one.
The framework thus transforms an informal sensitivity analysis into a
statistically grounded diagnostic.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{A Consequential Application: Cigarette Demand and the
Cross-Border Effect}
\label{subsec:empirical_cigar}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The Fama--French illustration deliberately reports ambiguity. We now turn
to a case in which the dependence profile changes an inferential
conclusion. We use the U.S. cigarette demand panel of \citet{Baltagi2006}, a
public dataset distributed with that text \citep{BaltagiCigarData}:
annual observations on $N=46$ states
over $T=30$ years (1963--1992), a standard testing ground for
cross-sectional dependence because cigarette markets are linked across
states by bootlegging and cross-border shopping. The data are public and
bundled with the replication package.

\paragraph{Regression and the contested coefficient.}
We estimate a conventional two-way (state and year) fixed-effects demand
equation,
\begin{equation}
\log \mathrm{sales}_{it}
=
\beta_1 \log p^{\mathrm{real}}_{it}
+
\beta_2 \log y^{\mathrm{real}}_{it}
+
\beta_3 \log p^{\mathrm{near}}_{it}
+
\alpha_i + \tau_t + u_{it},
\label{eq:cigar_regression}
\end{equation}
where $\mathrm{sales}_{it}$ is per-capita sales, $p^{\mathrm{real}}$ is
the real price, $y^{\mathrm{real}}$ is real per-capita income, and
$p^{\mathrm{near}}$ is the minimum real price in neighboring states. The
coefficient of interest is $\beta_3$: a negative value indicates that
cheaper cigarettes nearby draw sales away from a state---the cross-border
(bootlegging) effect that motivates much of the empirical
cigarette-tax literature. The price and income elasticities are estimated
sharply and are significant under every standard-error method
(Table~\ref{tab:cigar_se}); the cross-border effect is the coefficient
whose significance is in question.

\paragraph{The inferential problem.}
Table~\ref{tab:cigar_se} reports $\hat\beta_3$ with four standard errors.
The estimate is $\hat\beta_3=-0.117$ under all of them---only the
standard error changes---yet the conclusion does not survive that change.
Under homoskedastic and cluster-by-year standard errors the effect is
significant at the five percent level ($p=0.030$ and $p=0.041$); under
HC1 and the conventional cluster-by-state standard errors it is not
($p=0.064$ and $p=0.170$). A researcher who follows the common default of
clustering by state concludes that cross-border effects are absent; one
who allows for a common temporal shock concludes the opposite. Nothing in
the regression output adjudicates between them.

\begin{table}[htbp]
\centering
\caption{Cigarette demand: $\hat\beta$ and four standard errors. The
cross-border coefficient (log nearby min price) is significant at five
percent under homoskedastic and cluster-by-year standard errors, and
insignificant under HC1 and cluster-by-state.}
\label{tab:cigar_se}
\small
\inputIfExists{results/tables/table_cigar_standard_errors.tex}
\end{table}

\paragraph{What the dependence profile says.}
We estimate the profile on the two-way within residuals, using exactly the
operator of the rest of the paper: $\widehat\Gamma_T=T^{-1}\sum_t\widehat
u_t\widehat u_t'$ projected onto the cluster (four census regions), factor
($r=1$), and sparse ($10\%$ of off-diagonal pairs) geometries, estimated without
reference to which standard error is ``interesting.'' Table~\ref{tab:cigar_profile}
reports the result: the estimated \emph{full dependence profile} is
factor-dominant, $\widehat{\boldsymbol\omega}=(0.16,\,0.46,\,0.38)$, and the
\emph{off-diagonal dependence profile}---the object that drives procedure
selection---points the same way, since the factor geometry fits the residual
co-movement far better than the alternatives ($\widehat\rho_F=0.15$, well below
the cluster residual $\widehat\rho_C=0.81$). The confidence index is
$\widehat\kappa=0.07$---modest but, unlike the Fama--French case, backed by a
genuinely small $\widehat\rho_{\min}$: here the dictionary fits.

\begin{table}[htbp]
\centering
\caption{Cigarette demand: dependence profile and diagnostics for the
residual operator. Factor dependence dominates and fits well
($\widehat\rho_F=0.15$); cluster dependence fits poorly
($\widehat\rho_C=0.81$).}
\label{tab:cigar_profile}
\small
\inputIfExists{results/tables/table_cigar_profile.tex}
\end{table}

\paragraph{Interpretation.}
The profile indicates that what remains of the cross-sectional dependence after
two-way demeaning is factor-shaped rather than state-clustered, and this is
economically sensible. The factor cannot be a common additive year shock---
additive year effects $\tau_t$ are already absorbed by the within
transformation---but instead reflects \emph{heterogeneous exposure} to
nationally common forces: cigarette demand across states responds with differing
sensitivity to national anti-smoking campaigns, federal tax and regulatory
changes, nationally marketed advertising, and secular shifts in health attitudes.
States with similar demographics, smoking cultures, or regulatory environments
load similarly on these common movements, producing a low-rank co-movement in
residual demand that a single national dummy per year cannot absorb and that
within-state clustering is not designed to capture. This is exactly the
structure the factor geometry detects, which is why it both dominates the profile
and fits well ($\widehat\rho_F=0.15$) while the state-cluster geometry fits worst
($\widehat\rho_C=0.81$). Clustering by state, the conventional default, targets
within-state serial correlation that the profile finds both subdominant and
poorly fitting, and it is the method under which the cross-border effect appears
insignificant; standard errors that accommodate the common temporal factor keep
it significant. The profile thus provides evidence favoring the latter and
identifies the state-clustered standard error as the one whose maintained
assumption the data support least. Because $\widehat\kappa=0.07$ is modest, we
report all four procedures and treat the reading as a principled sensitivity
analysis rather than a definitive resolution.

\paragraph{From classical to adaptive inference.}
It is worth stating plainly what the framework changes here. \emph{Classical
practice} fixes a dependence assumption before looking at the residual
dependence---most commonly clustering by state---and reads off the standard
error it implies; under that default the cross-border coefficient is
insignificant ($p=0.170$), and the researcher concludes that bootlegging leaves
no detectable footprint. \emph{Adaptive inference} instead learns the dependence
geometry from the same residuals: the off-diagonal profile points to a factor
structure that fits well and away from the state-cluster structure that fits
poorly, directing inference to a common-shock--robust standard error under which
the same point estimate ($\widehat\beta_3=-0.117$) is significant ($p=0.030$).
The two routes reach \emph{opposite substantive conclusions} about a
policy-relevant elasticity from identical data and an identical coefficient; what
differs is only the maintained dependence assumption, and the classical route
selects that assumption by convention while the adaptive route selects it by
evidence. This is the concrete answer to ``why learn the geometry?''---not a
tighter standard error for its own sake, but protection against a default
dependence assumption that the data actively contradict.

\paragraph{Transparency.}
Two caveats are reported openly. First, because the operator is formed from
two-way within residuals with $T=30<N=46$, $\widehat\Gamma_T$ is rank-deficient
(rank $29$); this does not affect the profile, which is a projection functional
requiring no inverse of $\widehat\Gamma_T$. Second, the object profiled is the
dependence operator of the \emph{within-transformed} residuals: with $N$ fixed,
year demeaning applies the fixed linear map $M_N=I_N-N^{-1}\mathbf 1\mathbf 1'$
to each cross-section, so $\widehat\Gamma_T$ estimates $M_N\Sigma M_N$ rather
than $\Sigma$. This is the correct target, not a defect---the coefficient
estimator and all four standard errors are computed from the same
within-transformed data---and Proposition~\ref{prop:consistency_operator} applies
once $u_t$ is read as the within-transformed disturbance, via the generic
residual condition of Remark~\ref{rem:generic_residuals}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Cov_Learn_arxiv_v2/sections/estimation.tex <==
\section{Statistical Learning of Dependence Profiles}
\label{sec:estimation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

This section describes how the population dependence profile $\omega_0$
is estimated from data. The empirical dependence operator
$\widehat\Gamma_T$ was introduced in~\eqref{eq:sample_cov} and shown to
be consistent for $\Gamma_0$ in Proposition~\ref{prop:consistency_operator}.
Dependence profiles, projection-residual diagnostics, and their
sample counterparts are defined below.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Choice of Dependence Operator}
\label{subsec:operatorchoice}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The empirical operator $\widehat\Gamma_T$ should capture the dependence relevant
for the inferential problem: the residual covariance
operator~\eqref{eq:sample_cov} for contemporaneous cross-sectional dependence, a
long-run covariance operator under serial dependence, or distance-, adjacency-,
or cluster-based operators for spatial, network, or clustered data. The framework
does not select a unique operator; it studies the covariance geometry encoded in
a chosen $\Gamma_0$. The dependence profile is invariant to positive rescalings
of the operator; additional examples and technical details are in the Online
Appendix.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Projection-Residual Diagnostics}
\label{subsec:projection_residuals}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The dependence profile provides a relative measure of geometric fit.
To assess goodness-of-fit in an absolute sense, we introduce
projection-residual diagnostics.

Define the normalized projection residual
\[
\rho_d(\Gamma)
=
\frac{
\|
\Gamma-P_d(\Gamma)
\|_F
}
{
\|\Gamma\|_F
},
\qquad
d\in\mathfrak D,\ \Gamma\neq0.
\]
The quantity $\rho_d(\Gamma)$ measures the fraction of the operator
that remains unexplained after projection onto geometry $d$. Since
$0\in\mathcal S_d$, the definition of the projection implies
$\|\Gamma-P_d(\Gamma)\|_F\le\|\Gamma\|_F$, so $0\le\rho_d(\Gamma)\le1$.
Small values indicate that geometry $d$ provides a good approximation
to the dependence operator, whereas large values indicate substantial
lack of fit.

Define the minimum residual
\[
\rho_{\min}(\Gamma)
=
\min_{d\in\mathfrak D}
\rho_d(\Gamma).
\]
We say that a dependence operator exhibits a ``none-of-the-above''
pattern whenever $\rho_{\min}(\Gamma)>\delta$ for a prespecified
threshold $\delta\in(0,1)$. Large values of $\rho_{\min}$ indicate
that none of the cluster, factor, or sparse geometries provides an
adequate approximation to the observed dependence structure.

\begin{proposition}
\label{prop:residual_consistency}
Suppose Assumptions~\ref{ass:local_projection_regularity} and~\ref{ass:mixing} hold. Then
\[
\rho_d(\widehat\Gamma_T)
\overset{p}{\longrightarrow}
\rho_d(\Gamma_0),
\qquad
d\in\mathfrak D,
\]
and $\rho_{\min}(\widehat\Gamma_T)\overset{p}{\longrightarrow}
\rho_{\min}(\Gamma_0)$.
\end{proposition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Similarity-Score Estimation}
\label{subsec:similarity_score_estimation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Define the estimated projection, similarity score, and dependence
profile as
\[
\widehat P_d = P_d(\widehat\Gamma_T),
\qquad
\widehat S_d = \|\widehat P_d\|_F^2,
\qquad
\widehat\omega_d = \frac{\widehat S_d}{\sum_{d\in\mathfrak D}\widehat S_d},
\qquad d\in\mathfrak D.
\]
The estimated dependence profile is
$\widehat\omega=(\widehat\omega_C,\widehat\omega_F,\widehat\omega_S)'$.

The use of the projection \emph{magnitude} $\|P_d(\Gamma)\|_F^2$ rather
than the projection \emph{distance} $\|\Gamma-P_d(\Gamma)\|_F^2$ requires
justification, since the classes are nonconvex and the two are equivalent
only through a Pythagorean identity that is automatic for linear
subspaces but not for general sets. The following lemma supplies it.

\begin{lemma}[Conic Pythagoras]
\label{lem:conic_pythagoras}
Each geometry $\mathcal S_d$, $d\in\mathfrak D$, is a cone containing the
origin: $\Gamma\in\mathcal S_d$ and $a\ge 0$ imply $a\Gamma\in\mathcal
S_d$. Consequently, for every $\Gamma\in\mathbb H$ and every metric
projection $p=P_d(\Gamma)$,
\[
\langle \Gamma-p,\;p\rangle_F=0,
\qquad
\|\Gamma\|_F^2=\|P_d(\Gamma)\|_F^2+\|\Gamma-P_d(\Gamma)\|_F^2 .
\]
\end{lemma}

\noindent
The proof is in the Online Appendix.

\noindent
Lemma~\ref{lem:conic_pythagoras} shows that the similarity score and the
projection residual are two encodings of the same information:
\begin{equation}
S_d(\Gamma)=\|\Gamma\|_F^2\bigl(1-\rho_d(\Gamma)^2\bigr),
\qquad
\rho_d(\Gamma)=\frac{\|\Gamma-P_d(\Gamma)\|_F}{\|\Gamma\|_F},
\qquad \Gamma\neq0 .
\label{eq:score_residual_duality}
\end{equation}
In particular $S_i(\Gamma)>S_j(\Gamma)$ if and only if
$\|\Gamma-P_i(\Gamma)\|_F<\|\Gamma-P_j(\Gamma)\|_F$: ranking geometries by
projection magnitude is \emph{equivalent} to ranking them by
best-approximation distance, so the dominant geometry of
Section~\ref{sec:classification} is exactly the best-fitting geometry, and
no separate justification of the score is required.

\begin{lemma}[Diagonal invariance of the geometric ranking]
\label{lem:diagonal_invariance}
Suppose each projection reproduces the diagonal of its argument,
$\operatorname{diag}(P_d(\Gamma))=\operatorname{diag}(\Gamma)$ for all
$d\in\mathfrak D$. Then
\[
S_d(\Gamma)
=
\|\operatorname{diag}(\Gamma)\|_F^2
+
\|\operatorname{off}(P_d(\Gamma))\|_F^2 ,
\]
so the scores differ across geometries only through their off-diagonal
parts. Consequently the dominant geometry satisfies
$d^\star=\arg\max_d\|\operatorname{off}(P_d(\Gamma))\|_F^2$ and is
invariant to the diagonal of $\Gamma$.
\end{lemma}

\noindent
The proof is in the Online Appendix.

\noindent
The diagonal condition holds exactly for the cluster geometry (unit-diagonal
support) and the sparse geometry (off-diagonal thresholding), and for the factor
geometry whenever the idiosyncratic nonnegativity constraint is slack, since
$D=\operatorname{diag}(\Gamma-L)$ then reproduces $\operatorname{diag}(\Gamma)$.
When it holds for every geometry, the $S_d$ ranking depends only on off-diagonal
dependence, aligning classification with the principal-angle analysis. For the
factor geometry, when the constraint binds the diagonal can affect the
full-profile ranking, so the full and off-diagonal profiles need not rank
geometries identically. The off-diagonal profile is therefore a formal companion
estimand, not an optional robustness check:
\begin{equation}
S_d^{\mathrm{off}}(\Gamma)
=\|\operatorname{off}\{P_d(\Gamma)\}\|_F^2,
\qquad
\omega_d^{\mathrm{off}}(\Gamma)
=\frac{S_d^{\mathrm{off}}(\Gamma)}
{\sum_{j\in\mathfrak D}S_j^{\mathrm{off}}(\Gamma)},
\label{eq:off_profile}
\end{equation}
whenever the denominator is positive, with sample counterpart
\[
\widehat\omega_d^{\mathrm{off}}
=\frac{\|\operatorname{off}(\widehat P_d)\|_F^2}
{\sum_{j}\|\operatorname{off}(\widehat P_j)\|_F^2}.
\]
The full profile measures overall
covariance fit; the off-diagonal profile measures dependence architecture after
removing marginal variances. Classification and profile-guided inference use the
off-diagonal profile as the primary rule (the identification analysis is on the
off-diagonal tangent spaces), with the full profile as a companion diagnostic;
all consistency and delta-method results below apply jointly to
$(\omega,\omega^{\mathrm{off}})$ by stacking the two smooth score maps whenever
both denominators are positive.

\paragraph{Why the off-diagonal profile.}
It is natural to ask why geometry learning is based on
$\omega^{\mathrm{off}}$ rather than on the full profile $\omega$. The reason is
that the diagonal of the covariance operator carries \emph{marginal variance}
information that is common to all candidate geometries and largely uninformative
about which \emph{dependence} structure generated the data. Every geometry in the
dictionary reproduces (or nearly reproduces) $\operatorname{diag}(\Gamma)$, so the
diagonal contributes a common, geometry-invariant term
$\|\operatorname{diag}(\Gamma)\|_F^2$ to each score $S_d$. Including it in the
profile therefore adds the \emph{same} constant to every numerator, mechanically
pulling the full profile toward the uniform vector $(1/3,1/3,1/3)$ and
compressing exactly the differences across geometries that classification must
detect. This diagonal term also makes the full profile sensitive to the
\emph{scale} of individual series: rescaling one unit's disturbance inflates its
variance and hence its diagonal contribution, shifting $\omega$ without changing
the dependence pattern at all. The off-diagonal profile removes both effects. By
restricting the scores to $\operatorname{off}(P_d)$ it discards the common
diagonal term and the marginal variances, isolating the cross-sectional
co-movement that actually distinguishes clustering, factor, and sparse
dependence. This is also why the identification and impossibility results are
stated on the off-diagonal tangent spaces: it is there, not on the diagonal, that
two geometries either separate or overlap. The full profile is retained because
it answers a different and still useful question---how well the dictionary
approximates the entire operator, diagonal included---and because a large gap
between $\omega$ and $\omega^{\mathrm{off}}$ is itself a diagnostic that marginal
heterogeneity is masking the dependence geometry.

\begin{proposition}[Joint consistency of full and off-diagonal profiles]
\label{prop:joint_profile_consistency}
Under Assumptions~\ref{ass:local_projection_regularity}
and~\ref{ass:mixing}, and if both normalizing denominators are positive,
then
\[
(\widehat\omega-\omega_0,
 \widehat\omega^{\mathrm{off}}-\omega_0^{\mathrm{off}})
=O_p(T^{-1/2}).
\]
Under Assumptions~\ref{ass:operatorclt}
and~\ref{ass:projection_differentiability}, and the same positivity
conditions,
\[
\sqrt T
\begin{pmatrix}
\widehat\omega-\omega_0\\
\widehat\omega^{\mathrm{off}}-\omega_0^{\mathrm{off}}
\end{pmatrix}
\Rightarrow N(0,\Xi_{\mathrm{joint}}),
\]
where $\Xi_{\mathrm{joint}}$ is obtained by applying the stacked
full- and off-diagonal-profile Jacobian to $\Omega_\Gamma$.  We write
$\Xi_{\mathrm{off}}$ for its off-diagonal-profile marginal block.
\end{proposition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Cov_Learn_arxiv_v2/sections/geometry.tex <==
\section{Statistical Experiment, Estimability, and Covariance Geometry}
\label{sec:geometry}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Statistical Experiment}
\label{subsec:stat_experiment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let $N\geq 1$ denote the cross-sectional dimension, treated as fixed
throughout. We observe a panel
\[
\{u_t\}_{t=1}^T,
\qquad u_t=(u_{1t},\ldots,u_{Nt})'\in\mathbb R^N,
\]
where $u_t$ is a zero-mean random vector with covariance matrix
\[
\Sigma = E(u_t u_t') \in \mathbb{R}^{N\times N}.
\]
Asymptotics are driven by the time dimension: $T\to\infty$ with $N$
fixed.

\begin{remark}[Asymptotic regime]
\label{rem:asymptotic_regime}
Throughout, $N$ is fixed and $T\to\infty$. The cross-sectional dimension $N$
governs the \emph{geometry} of dependence---the dimension of the Hilbert space,
the projection operators, and the principal-angle conditions---while $T$ governs
\emph{estimation}, the rate at which the empirical operator concentrates around
its population counterpart. This separation between the geometric and asymptotic
dimensions is what makes the framework well-posed.
\end{remark}

\subsection{Population Dependence Operator}
\label{subsec:pop_dep_operator}

We equip the space of symmetric $N\times N$ matrices with the Frobenius
inner product
\[
\langle A, B\rangle_F = \operatorname{tr}(A'B),
\qquad
\|A\|_F = \langle A,A\rangle_F^{1/2},
\]
giving the Hilbert space
\[
\mathbb{H} = \bigl\{A\in\mathbb{R}^{N\times N}: A=A',\;\|A\|_F<\infty\bigr\}.
\]

\begin{definition}[Population Dependence Operator]
\label{def:pop_dep_op}
The \emph{population dependence operator} is the element
$\Gamma_0\in\mathbb{H}$ represented by the covariance matrix
\[
\Gamma_0 \;=\; \Sigma \;=\; E(u_t u_t').
\]
\end{definition}

\noindent
The Hilbert-space formulation in Definition~\ref{def:pop_dep_op} is not
merely notational. Representing $\Sigma$ as an element of
$(\mathbb{H},\langle\cdot,\cdot\rangle_F)$ enables the use of
projection operators, tangent spaces, and principal angles---the central
geometric objects of the paper. In finite dimensions, $\Gamma_0$ is
identified with $\Sigma$; in extensions to functional or network data,
the same abstract framework accommodates more general covariance kernels
or operators without changing the theoretical results.

\subsection{Empirical Dependence Operator and Estimability}
\label{subsec:estimability}

We observe $T$ cross-sectional vectors $u_1,\ldots,u_T$. In practice $u_t$ is
typically not observed directly but recovered as residuals from a regression
model; the leading case, used in the simulation and empirical sections, is the
panel regression
\begin{equation}
y_{it} = x_{it}'\beta + u_{it},
\qquad i=1,\ldots,N,\quad t=1,\ldots,T,
\label{eq:panel_regression}
\end{equation}
with $u_t=(u_{1t},\ldots,u_{Nt})'$ and $\widehat\Gamma_T$ built from the OLS
residuals $\widehat u_t$. The estimand is $\Gamma_0=\Sigma=E(u_tu_t')$, a fixed
$N\times N$ positive semidefinite matrix: since $N$ is fixed, this is not the
problem of estimating a covariance matrix that grows with the sample, but of
estimating a fixed matrix using an increasing number of time-series
observations. The natural estimator is the sample covariance of the (estimated)
residuals,
\begin{equation}
\widehat\Gamma_T
=
\frac{1}{T}
\sum_{t=1}^{T}
\widehat u_t\widehat u_t',
\label{eq:sample_cov}
\end{equation}
$\widehat u_t = (\widehat u_{1t},\ldots,\widehat u_{Nt})'$. We state the formal
conditions and consistency as a proposition, giving the estimator an explicit
foundation before the geometric theory.

\begin{assumption}[Stationarity, Mixing, and Moments]
\label{ass:mixing}
The joint process $\{(u_t,X_t)\}$ is strictly stationary and ergodic,
where $X_t\in\mathbb{R}^{N\times p}$ collects the regressors at time
$t$. There exists $\delta>0$ such that $E\|u_t\|^{4+\delta}<\infty$
and $E\|X_t\|_F^{2+\delta}<\infty$. The mixing condition is imposed
directly on the \emph{quadratic} process
$\psi_t=\operatorname{vec}(u_tu_t'-\Sigma)$, which is the process to
which the central limit theorem is applied: writing $\eta=\delta/2$, so
that $E\|\psi_t\|^{2+\eta}<\infty$ whenever
$E\|u_t\|^{4+\delta}<\infty$, the process satisfies strong mixing with
\[
\sum_{k=0}^\infty \alpha(k)^{\eta/(2+\eta)}
=
\sum_{k=0}^\infty \alpha(k)^{\delta/(4+\delta)}
<\infty ,
\]
where $\alpha(k)$ is the strong mixing coefficient of
$\{(u_t,X_t)\}$ at lag $k$ (mixing coefficients of $\{\psi_t\}$ are
bounded by those of $\{u_t\}$, since $\psi_t$ is a measurable function of
$u_t$). This is the summability exponent required by the mixing central
limit theorem applied to $\{\psi_t\}$, and it is the binding condition;
the more familiar exponent $\delta/(2+\delta)$ would be appropriate for
$\{u_t\}$ itself rather than for the quadratic process.
The regressors are strictly exogenous, the OLS estimator satisfies
$\hat\beta-\beta=O_p(T^{-1/2})$, and the regressor--error cross
moment obeys
\[
\frac1T\sum_{t=1}^T X_t\otimes u_t=O_p(T^{-1/2}).
\]
The last rate is the condition used to make residual replacement
first-order negligible; it follows, for example, from an appropriate
mixing central limit theorem for the cross-product process. In particular,
$T^{-1}\sum_{t=1}^T\|X_t\|_F^2=O_p(1)$ by the ergodic theorem.
\end{assumption}

\begin{proposition}[Consistency of the Empirical Dependence Operator]
\label{prop:consistency_operator}
Under Assumption~\ref{ass:mixing},
\[
\|\widehat\Gamma_T - \Gamma_0\|_F = O_p(T^{-1/2}).
\]
\end{proposition}

\begin{remark}[Generic residual constructions]
\label{rem:generic_residuals}
Assumption~\ref{ass:mixing} describes a fixed-dimensional, common-$\beta$ OLS
problem. Empirical designs often use richer residual constructions---most
commonly a two-way within transformation---not covered directly, so it is useful
to state the requirement generically. Let $\widehat u_t$ be any residual
construction and $u_t$ the corresponding population disturbance, and suppose
\[
\frac1T\sum_{t=1}^T(\widehat u_t-u_t)(\widehat u_t-u_t)'=O_p(T^{-1}),
\qquad
\frac1T\sum_{t=1}^T(\widehat u_t-u_t)u_t'=O_p(T^{-1}),
\tag{R}
\label{eq:generic_residual}
\]
together with the stationarity, moment, and mixing conditions of
Assumption~\ref{ass:mixing} imposed on $\{u_t\}$. Then the conclusion of
Proposition~\ref{prop:consistency_operator} holds verbatim and, by
Remark~\ref{rem:primitive_clt}, the influence function is unchanged.
Condition~\eqref{eq:generic_residual} is verified for common-$\beta$ OLS under
strict exogeneity in the proof of Proposition~\ref{prop:consistency_operator}.
For a two-way fixed-effects specification, the relevant transformed disturbance
and its covariance operator must be defined from the complete within
transformation, and \eqref{eq:generic_residual} verified for that construction;
with fixed $N$ this is standard under suitable moment, exogeneity, and
weak-dependence conditions, but it is design-specific and not an automatic
consequence of Proposition~\ref{prop:consistency_operator}. Researchers using
other constructions should verify~\eqref{eq:generic_residual} directly.
\end{remark}

\noindent
Proposition~\ref{prop:consistency_operator} confirms that $\Gamma_0$ is a
well-defined, consistently estimable estimand at the $\sqrt T$-rate that drives
all the CLTs of Section~\ref{sec:asymptotics}. The proof decomposes
$\widehat\Gamma_T-\Gamma_0$ into the sampling error of the infeasible covariance
$T^{-1}\sum_t u_tu_t'$ (which is $O_p(T^{-1/2})$ under Assumption~\ref{ass:mixing}
by standard results for weakly dependent processes, e.g.\
\citealt{Davidson1994}) and a residual-replacement remainder that is
$O_p(T^{-1})$ under strict exogeneity. Estimating $\Gamma_0$ is not the goal in
itself: $\widehat\Gamma_T$ is an intermediate object from which the estimand of
interest, the population profile $\omega_0$, is constructed.

\begin{remark}[Two notions of dependence]
\label{rem:two_dependence_notions}
The weak-dependence conditions on $\{u_t\}$ in
Proposition~\ref{prop:consistency_operator} concern the \emph{temporal} sequence
across $t$ and serve only to guarantee consistent estimation of $\Gamma_0$; they
place \emph{no} restriction on the \emph{cross-sectional} dependence structure
encoded in $\Gamma_0=E(u_tu_t')$, which is precisely the object being learned.
Temporal and cross-sectional dependence are therefore distinct, and assumptions
on the former do not restrict the latter.
\end{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Covariance Classes}
\label{subsec:cov_classes}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Rather than assuming $\Gamma_0$ belongs to a single class, we characterize its
dependence architecture through geometric proximity to several economically
meaningful covariance classes. Each geometry, defined next, is a
\emph{deterministic} subset of $\mathbb H$, so the projection of $\Gamma_0$ onto
it is well defined. Let $\mathcal S_C,\mathcal S_F,\mathcal S_S$ denote the
cluster, factor, and sparse classes.

\begin{definition}[Covariance-cone dictionary]
\label{def:covariance_cone_dictionary}
Write $\mathbb H_+=\{\Gamma\in\mathbb H:\Gamma\succeq0\}$.  Every
candidate geometry used in this paper is a nonempty closed cone contained
in $\mathbb H_+$.  Consequently every projected point is itself a valid
covariance matrix.  This restriction is substantive: the dictionary
classifies covariance structure, rather than merely symmetric support
patterns.
\end{definition}

For a prespecified cluster-support matrix $M_C$ with unit diagonal, define
\[
\mathcal S_C
=
\{\Gamma\in\mathbb H_+:\Gamma_{ij}=0\text{ whenever }(M_C)_{ij}=0\}.
\]
Thus the cluster class is the intersection of the covariance cone with a
fixed linear support space.  It is a closed convex cone.  For one-way
partitions the support mask is block diagonal and masking preserves
positive semidefiniteness.  For overlapping multiway supports the metric
projection is the solution of a convex PSD-constrained least-squares
problem; entrywise masking alone is not, in general, the metric
projection.

The support matrix is constructed from the clustering dimensions by
\[
(M_C)_{ij}
=
\ind\Bigl\{g_m(i)=g_m(j)\text{ for at least one }m\in\{1,\ldots,M\}\Bigr\}.
\]
This includes one-way, two-way, and multiway cluster dictionaries.

\begin{remark}[Cluster geometry versus many-cluster asymptotics]
\label{rem:cluster_vs_manycluster}
The paper's objective is not the asymptotic validity of cluster-robust variance
estimators under many-cluster asymptotics. The cluster covariance class here is a
finite-dimensional geometry on a fixed $N\times N$ matrix describing which entries
are compatible with a given one-way, two-way, or multiway support---distinct from
the many-cluster theory used to justify conventional cluster-robust standard
errors. The present fixed-$N$, $T\to\infty$ framework studies learning the
cross-sectional geometry; validity of a particular geometry-specific inference
action is imposed separately when that action is used.
\end{remark}

For a fixed rank $r$, define the factor class as
\[
\mathcal S_F(r)
=
\Big\{
\Gamma\succeq0:
\Gamma=L+D,\;
L\succeq0,\;
\operatorname{rank}(L)\le r,\;
D\succeq0 \text{ diagonal}
\Big\}.
\]

For a fixed sparsity budget $k_S\le N(N-1)/2$, define the sparse
covariance cone as
\[
\mathcal S_S
=
\Big\{
\Gamma\in\mathbb H_+:
|\operatorname{supp}_{\mathrm{off}}(\Gamma)|\le k_S
\Big\},
\]
where $\operatorname{supp}_{\mathrm{off}}(\Gamma)=\{(i,j):i<j,
\Gamma_{ij}\neq0\}$.  This is a finite union of closed convex cones and
is therefore a closed, generally nonconvex cone.  Its exact metric
projection jointly selects a support and solves a PSD-constrained
least-squares problem on that support.  The computational appendix uses
a transparent support-selection plus constrained-refinement algorithm;
the population theory concerns the exact metric projection.

The dictionary is intentionally illustrative rather than exhaustive: the
framework extends to any family of closed covariance geometries satisfying the
projection regularity assumptions. Cluster, factor, and sparse geometries are
adopted because they encompass the most widely used dependence structures in
econometric practice---group-correlated shocks, pervasive common variation, and
localized or network linkages. A researcher who suspects an additional structure
may enlarge the dictionary by adding the corresponding closed class, with no
change to the identification, impossibility, or adaptive-inference theory,
provided the new class admits a well-defined projection.

\subsection{Projection Operators}
\label{subsec:projections}

Throughout the paper, let
\[
\mathfrak D=\{C,F,S\}
\]
denote the covariance-cone dictionary, corresponding respectively to
cluster, factor, and sparse dependence. Define
\[
P_d(\Gamma)
=
\arg\min_{\Gamma'\in\mathcal S_d}
\|\Gamma-\Gamma'\|_F.
\]
$P_d(\Gamma)$ represents the closest approximation to $\Gamma$ within
the covariance class $\mathcal S_d$. Although we use projection
notation, $P_d$ need not be a linear orthogonal projection because the
covariance classes may be nonlinear or nonconvex.

\begin{lemma}[Existence of Projections]
\label{lem:projectionexistence}
If $\mathcal S_d$ is closed in $\mathbb H$, then $P_d(\Gamma)$ exists
for every $\Gamma\in\mathbb H$.
\end{lemma}

\begin{lemma}[Continuity of Projection Operators]
\label{lem:projectioncontinuity}
Suppose $P_d$ is locally unique at $\Gamma$. If $\Gamma_m\to\Gamma$,
then $P_d(\Gamma_m)\to P_d(\Gamma)$.
\end{lemma}

\subsection{Why the Frobenius Geometry?}
\label{subsec:frobenius}

The Frobenius norm is induced by the Hilbert inner product
$\langle A,B\rangle_F=\operatorname{tr}(A'B)$ and therefore provides a natural
geometry for projections, tangent spaces, principal angles, and local
separation. It is also computationally convenient: low-rank projections use
spectral updates, one-way cluster projections reduce to block support masks, and
general cluster or sparse projections reduce to PSD-constrained fixed-support
least squares (with support selection for sparse classes). Alternative metrics
may suit other applications, but the Frobenius geometry gives the most
transparent framework for the theory below.


\subsection{Dependence Profile}
\label{subsec:dep_profile}

Define the \emph{population similarity score} for geometry $d$ as
\[
S_{d,0}=\|P_d(\Gamma_0)\|_F^2,
\qquad d\in\mathfrak D.
\]
The normalized dependence similarity scores are
\[
\omega_{d,0}=\frac{S_{d,0}}{\sum_{d\in\mathfrak D}S_{d,0}},
\qquad d\in\mathfrak D.
\]
The vector
\[
\omega_0=(\omega_{C,0},\omega_{F,0},\omega_{S,0})'
\]
is called the \emph{population dependence profile}. It is a functional
of the estimable object $\Gamma_0$ and therefore inherits its
estimability from Proposition~\ref{prop:consistency_operator}.

\begin{remark}[No Variance Decomposition]
\label{rem:no_variance_decomp}
The quantities $\omega_{C,0},\omega_{F,0},\omega_{S,0}$ should not be
interpreted as fractions of covariance explained. Since the covariance
geometries overlap and the projections are not generally orthogonal,
$\sum_{d\in\mathfrak D}S_{d,0}\neq\|\Gamma_0\|_F^2$ in general. The
dependence profile measures relative geometric similarity, not additive
covariance contributions.
\end{remark}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Cov_Learn_arxiv_v2/sections/identification.tex <==
\section{Identification of Dependence Geometry}
\label{sec:identification}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
This section studies whether the dependence profile is well defined and
whether distinct covariance geometries are locally separated. The first
question is governed by regularity of the individual metric projections;
the second depends on whether the cluster, factor, and sparse geometries
have distinct local off-diagonal directions near the projected population
points.

Identification concerns the population operator; estimation concerns its
empirical counterpart. The identification theory of this section
therefore studies properties of $\Gamma_0$ and its projections,
independently of sampling variability.

For each $d\in\mathfrak D$, let
\[
\Sigma_d = P_d(\Gamma_0)
\]
denote the population projection of $\Gamma_0$ onto geometry $d$.
For each geometry \(d\in\mathfrak D\), let \(T_d(\Sigma_d)\) denote the
corresponding tangent space at this projected population point.
Since diagonal perturbations are common to all covariance geometries and
carry no information about cross-sectional dependence, identification is
based on the off-diagonal tangent spaces

\[
T_d^{\mathrm{off}}(\Sigma_d)
=
\left\{
H\in T_d(\Sigma_d)
:
H_{ii}=0
\ \text{for all } i
\right\},
\qquad
d\in\mathfrak D.
\]
\paragraph{Principal-Angle Condition.}
For two tangent spaces \(U\) and \(V\), define the smallest principal angle by
\[
\theta(U,V)
=
\arccos
\left(
\sup_{\substack{u\in U,\;v\in V\\ \|u\|_F=\|v\|_F=1}}
\bigl|\langle u,v\rangle_F\bigr|
\right),
\]
with the convention $\theta(U,V)=\pi/2$ if $U=\{0\}$ or $V=\{0\}$.

\begin{assumption}[Principal-Angle Identification]
\label{ass:principalangle}
There exists \(\theta_0>0\) such that
\[
\theta\bigl(T_i^{\mathrm{off}}(\Sigma_i),\,T_j^{\mathrm{off}}(\Sigma_j)\bigr)\ge \theta_0
\]
for all \(i\neq j\), \(i,j\in\mathfrak D\).
\end{assumption}
Formal definitions of the covariance geometries, regularity conditions,
and tangent spaces are given in the Online Appendix.


\begin{assumption}[Sparse Projection Regularity]
\label{ass:sparse_unique}

Let $\mathfrak I_S$ denote the finite collection of admissible symmetric
off-diagonal supports with cardinality at most $k_S$, and let
$\mathcal C_I=\{\Gamma\succeq0:\operatorname{supp}_{\mathrm{off}}(\Gamma)
\subseteq I\}$. The population sparse projection has a unique active
support $I_0$: there exists $\varepsilon_S>0$ such that
\[
\operatorname{dist}^2(\Gamma_0,\mathcal C_I)
\ge
\operatorname{dist}^2(\Gamma_0,\mathcal C_{I_0})+\varepsilon_S,
\qquad I\in\mathfrak I_S,\ I\neq I_0.
\]
This objective-gap condition, rather than an ordering of raw entries, is
the appropriate support-stability condition once positive
semidefiniteness is imposed.

\end{assumption}

\begin{lemma}[Principal Angle and Tangent-Space Transversality]
\label{lem:angle_transversality}
Let $U$ and $V$ be closed linear subspaces of $\mathbb H$. Then
$\theta(U,V)>0$ if and only if $U\cap V=\{0\}$.
\end{lemma}


\begin{theorem}[Well-Defined Dependence Profiles and Pairwise Geometric
Separation]
\label{thm:identification}
Suppose $\sum_{d\in\mathfrak D}S_{d,0}>0$ and the projected points
$\Sigma_d=P_d(\Gamma_0)$ are regular points at which the projections are
locally single-valued and continuous (Assumption~\ref{ass:sparse_unique}
for the sparse geometry). Then:
\begin{enumerate}
\item[(i)] \emph{(Well-definedness.)} The map
$\Gamma\mapsto\omega(\Gamma)=(\omega_C,\omega_F,\omega_S)(\Gamma)$ is
single-valued and continuous in a neighborhood of $\Gamma_0$; in
particular $\omega(\Gamma_0)$ is a well-defined functional of the
population dependence operator and is estimable at the rate of
Theorem~\ref{thm:profile_consistency}.
\item[(ii)] \emph{(Pairwise tangent separation.)} If in addition
Assumption~\ref{ass:principalangle} holds, then for every $i\neq j$ the
off-diagonal tangent spaces at the corresponding projected points
intersect trivially,
\[
T_i^{\mathrm{off}}(\Sigma_i)\cap T_j^{\mathrm{off}}(\Sigma_j)=\{0\}.
\]
\end{enumerate}
\end{theorem}

\begin{remark}[What Theorem~\ref{thm:identification} does and does not
assert]
\label{rem:identification_scope}
Part~(i) is a statement of well-definedness and estimability, not of
injectivity: because $\omega$ takes values in the two-dimensional simplex
while $\mathbb H$ has dimension $N(N+1)/2$, the profile map cannot be
locally injective on a full neighborhood of $\Gamma_0$, and no such claim
is made. The profile is a deliberate low-dimensional summary; the
projection residuals $\rho_d$ record what it discards.

Part~(ii) asserts pairwise trivial intersection only. A positive
principal angle means the tangent spaces do not intersect; it does not
make them orthogonal, so a perturbation lying in $T_i^{\mathrm{off}}$ may
still have a nonzero projection onto $T_j^{\mathrm{off}}$ and move more
than one score to first order. Nor do pairwise trivial intersections
imply a direct-sum decomposition when three or more geometries are
present---three distinct lines in a plane intersect pairwise trivially
without spanning independently. Attributing a first-order profile change
to a \emph{unique} geometry therefore requires the strictly stronger
condition that
$T_C^{\mathrm{off}}\oplus T_F^{\mathrm{off}}\oplus T_S^{\mathrm{off}}$ be
a direct sum on the relevant perturbation space, or equivalently that the
Jacobian of the score vector have full rank; we do not impose it and do
not claim unique attribution. What Assumption~\ref{ass:principalangle}
delivers, and what the subsequent theory uses, is that distinct
geometries are locally distinguishable in the pairwise sense of~(ii). The
complementary configuration, in which two geometries share a common point
\emph{and} a common tangent direction, is exactly the source of the
fundamental limit in Theorem~\ref{thm:fundamental_limit}.
\end{remark}

\begin{assumption}[Local Asymptotic Normality]
\label{ass:lan}
Let $P_\Gamma^T$ denote the joint distribution of $(u_1,\ldots,u_T)$
when the cross-sectional covariance matrix is $\Gamma$. The statistical
model $\{P_\Gamma^T:\Gamma\in\mathbb H\}$ satisfies local asymptotic
normality (LAN) at $\Gamma_0$, \emph{uniformly over bounded local
perturbations}: for every bounded sequence $H_T\to H$ in $\mathbb H$, with
the $o_p(1)$ remainder below uniform over $\|H\|_{\mathcal I}\le B$ for
each fixed $B<\infty$,
\[
\log\frac{dP_{\Gamma_0+T^{-1/2}H_T}^T}{dP_{\Gamma_0}^T}
=
\frac{1}{\sqrt T}\sum_{t=1}^T \ell_t(H)
-
\tfrac12\|H\|_{\mathcal I}^2
+o_p(1),
\]
where $\ell_t(H)$ is a zero-mean score with $E[\ell_t(H)^2]=\|H\|_{\mathcal I}^2$ for
a positive-definite inner product $\|\cdot\|_{\mathcal I}$ on $\mathbb H$.
The local perturbations $\Gamma_0+T^{-1/2}H_T$ are required to be
positive semidefinite and to belong to the parameter space for all
sufficiently large $T$; when $\Gamma_0$ is positive definite this holds
for every fixed $H\in\mathbb H$, and otherwise $H$ is restricted to
admissible tangent directions.
In addition, the local experiment is asymptotically continuous in
Hellinger distance: for any bounded local sequences $H_T$ and $G_T$ with
$\|H_T-G_T\|_{\mathcal I}\to0$,
\[
H\!\left(
P_{\Gamma_0+T^{-1/2}H_T}^T,\,
P_{\Gamma_0+T^{-1/2}G_T}^T
\right)\to0.
\]
This property follows from differentiability in quadratic mean in the
regular finite-dimensional covariance experiments for which LAN is
invoked.
\end{assumption}
Assumption~\ref{ass:lan} is imposed only for the local impossibility
result (Theorem~\ref{thm:fundamental_limit}). It holds in regular
finite-dimensional covariance models, for example Gaussian experiments
with covariance parameter $\Gamma$; see \citet{LeCamYang2000},
Chapter~7. The assumption should be interpreted as a local regularity
condition on the statistical experiment at $\Gamma_0$, not as an
additional parametric restriction on the cross-sectional covariance
geometry being learned.
\subsection{Fundamental Limits of Dependence Learning}
The next result shows that ambiguity in dependence learning is not merely a
finite-sample phenomenon: when two geometries share a common off-diagonal tangent
direction, the data contain no first-order information distinguishing them along
local alternatives, so near-ties should be read as intrinsic ambiguity at the
relevant local scale rather than procedure failure.

\begin{theorem}[Fundamental limit of dependence learning]
\label{thm:fundamental_limit}
Let $\mathcal S_i$ and $\mathcal S_j$ be two covariance geometries with
$i\neq j$.
Suppose Assumption~\ref{ass:lan} holds at a regular point
$\Gamma_0\in\mathcal S_i\cap\mathcal S_j$, so that
$P_i(\Gamma_0)=P_j(\Gamma_0)=\Gamma_0$ and the off-diagonal tangent
spaces $T_i^{\mathrm{off}}(\Gamma_0)$, $T_j^{\mathrm{off}}(\Gamma_0)$
are evaluated at $\Gamma_0$ itself. Suppose there exists a nonzero
off-diagonal direction
$H \in T_i^{\mathrm{off}}(\Gamma_0)\cap T_j^{\mathrm{off}}(\Gamma_0)$.
 
Let $\Gamma_{i,T}\in\mathcal S_i$ and $\Gamma_{j,T}\in\mathcal S_j$ satisfy
\[
\Gamma_{i,T}
=
\Gamma_0+\frac{1}{\sqrt T}H+o(T^{-1/2}),
\qquad
\Gamma_{j,T}
=
\Gamma_0+\frac{1}{\sqrt T}H+o(T^{-1/2}).
\]
 
Then, for any sequence of tests $\varphi_T\in[0,1]$,
\[
\limsup_{T\to\infty}
\bigl|E_{\Gamma_{i,T}}\varphi_T-E_{\Gamma_{j,T}}\varphi_T\bigr|
=0.
\]
Consequently, no test can have asymptotic size tending to zero and power
tending to one for distinguishing $\mathcal S_i$ from $\mathcal S_j$ along
these local sequences.
\end{theorem}

Theorem~\ref{thm:fundamental_limit} establishes \emph{pairwise local
indistinguishability}: along these local sequences every test has asymptotically
identical rejection probability under the two geometries, so no classifier
separates them with non-trivial asymptotic power. We deliberately do not describe
this as a minimax lower bound---no quantified minimax risk bound is proved---but
as an impossibility statement along specified local sequences, which is what the
subsequent theory uses. It explains why the profile is deliberately continuous
rather than a hard model-selection device.

\begin{remark}[Identification versus Ambiguity]
\label{rem:identification_vs_ambiguity}
Theorems~\ref{thm:identification} and
\ref{thm:fundamental_limit} characterize the boundary between identifiable and ambiguous dependence
structures. Positive principal angles imply pairwise local separation of
the geometries, whereas overlapping tangent spaces imply local
indistinguishability.

\end{remark}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Cov_Learn_arxiv_v2/sections/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Introduction Part A — The inferential problem first
Applied researchers routinely face a consequential choice before conducting
inference: which dependence structure should govern the construction of
standard errors and critical values? Cluster-robust procedures require a
clustering partition \citep{LiangZeger1986,Arellano1987,CameronGelbachMiller2011,
CameronMiller2015}; factor-based corrections require a specification of the
latent factor structure \citep{Bai2003,ChamberlainRothschild1983}; and HAC,
spatial, and network procedures require a bandwidth, kernel, distance metric,
or network architecture \citep{White1980,NeweyWest1987,Andrews1991,Conley1999,
DriscollKraay1998,Auerbach2019,Leung2022}. These methods answer how to conduct
inference conditional on a dependence model. They do not answer the prior
question that arises when the relevant dependence model is itself unknown.

That prior question is empirically important. Firms may share industry shocks,
latent macroeconomic factors, and localized network linkages at the same time.
Regional outcomes may reflect institutional clustering together with spatial
spillovers. Financial returns may contain pervasive common components and
sparse pairwise interactions. Choosing one robust procedure by assumption can
therefore be difficult to justify and can materially affect empirical
conclusions. The statistical problem studied in this paper is consequently not
another variance-estimation problem under a maintained dependence structure.
It is the problem of learning the dependence structure that is most relevant
for inference and translating that evidence into a defensible inferential
decision.

We develop a unified framework for this problem. We observe a panel
$\{u_t\}_{t=1}^T$ of $N$-dimensional cross-sectional vectors, or residuals
thereof, with fixed $N$ and $T\to\infty$, so the covariance operator
$\Gamma_0=E(u_tu_t')$ is estimable. Rather than assuming $\Gamma_0$ belongs to
one covariance class, we compare it with a researcher-specified dictionary of
economically meaningful geometries---in the benchmark, cluster, factor, and
sparse covariance cones. Metric projections produce similarity scores whose
normalization forms a low-dimensional \emph{geometric dependence profile}: the
full profile records overall covariance fit, and an off-diagonal companion
isolates the cross-sectional dependence relevant for choosing among robust
procedures. The profile is a diagnostic, not a claim that the data reveal a
unique structural mechanism---it summarizes the relative support the operator
assigns to the dictionary, while projection residuals reveal when the dictionary
is inadequate and geometric overlap reveals when the data cannot discriminate
among its elements.

The resulting data-to-decision procedure has four linked components: the
operator is estimated and projected onto the candidate geometries; the profile
and residuals diagnose dominance, ambiguity, and dictionary misspecification;
geometric separation determines whether the dominant geometry is learnable; and
the learned geometry is mapped into an inference procedure through a decision
rule---recommending the matched procedure when one geometry dominates, reporting
ambiguity and supporting hybrid procedures near a tie, and warning against
geometry-specific inference when every projection fits poorly. Dependence is
therefore treated as an estimand, and adaptive inference becomes the prescriptive
consequence of learning it.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Introduction Part B — Theoretical contributions
The central theoretical question is whether the profile can reliably learn a
dominant geometry from an estimated dependence operator. The answer depends on
local projection regularity and on the geometric separation of the candidate
covariance classes. Principal angles between their off-diagonal tangent
directions measure separation between local approximations to the candidate
geometries. Positive angles provide pairwise local separation, whereas shared
tangent directions generate first-order indistinguishability. The same
geometric construction therefore characterizes both the circumstances under
which dependence learning is informative and the circumstances under which
reliable discrimination is impossible.

This yields a fundamental limit of dependence learning: near regions of
geometric overlap, no statistical procedure can distinguish competing
dependence structures at first order. Ambiguous dependence profiles
therefore reflect intrinsic nonidentification rather than finite-sample
uncertainty.

Beyond relative comparisons among candidate geometries, the framework
provides diagnostics for assessing the adequacy of the covariance
dictionary itself. Projection-residual diagnostics measure the distance
between the empirical dependence operator and its closest geometric
approximation, distinguishing three practically important situations: a
clearly dominant geometry, intrinsic ambiguity, and a misspecified
dictionary.

The inferential payoff is naturally decision theoretic \citep{Wald1950}.
Different robust procedures have different losses across dependence
geometries, so the empirical problem is procedure selection under uncertainty
about the dependence state. Existing methods typically resolve that
uncertainty by assumption before inference begins. We instead let the estimated
off-diagonal profile generate a data-driven decision rule. When its dominant
geometry is uniquely separated and profile rankings are compatible with
inferential loss, the selected procedure is asymptotically equivalent to an
infeasible oracle that knows the relevant geometry in advance and its regret
vanishes asymptotically. Thus the descriptive problem of dependence learning
and the prescriptive problem of inference selection are two stages of one
statistical decision problem.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Introduction Part C — Five contributions
The paper contributes to the literature in five ways.

\medskip

\noindent
\textbf{First}, we introduce a geometric framework for dependence
learning. We observe a panel and estimate the cross-sectional covariance
matrix $\Gamma_0$, which is a fixed $N\times N$ object consistently
estimable as $T\to\infty$. Covariance geometries are defined as closed covariance cones contained in the positive-semidefinite cone of the Hilbert space $(\mathbb{R}^{N\times N},\langle\cdot,
\cdot\rangle_F)$, and the dependence profile is obtained by projecting
the estimated $\hat\Gamma_T$ onto each candidate geometry. This
provides a unified representation of cluster, factor, sparse, and more
general dependence structures within a common mathematical framework.

\medskip

\noindent
\textbf{Second}, we establish an identification theory for dependence
learning. Under local projection regularity, dependence profiles are well defined; a principal-angle separation condition establishes pairwise separation of the candidate geometries. Under additional sampling and projection-%
differentiability conditions, the full and off-diagonal profiles are consistently estimable and asymptotically normal. We further derive finite-sample classification
error bounds that quantify the reliability of dependence learning.

\medskip

\noindent
\textbf{Third}, we characterize the fundamental limits of dependence
learning. We show that when covariance geometries share common tangent
directions, no statistical procedure can distinguish them at first
order. This impossibility theorem demonstrates that ambiguous
dependence profiles may reflect intrinsic nonidentification rather than
finite-sample uncertainty; projection-residual diagnostics complement
these results by testing whether the candidate dictionary itself is
adequate.

\medskip

\noindent
\textbf{Fourth}, we develop a framework for adaptive econometric
inference under unknown dependence. Estimated off-diagonal dependence profiles guide
the selection of dependence-robust inference procedures. Under a unique
profile margin and an explicit profile--loss compatibility condition, the
selected procedure is asymptotically equivalent to an infeasible oracle
possessing prior knowledge of the dominant dependence structure.

\medskip

\noindent
\textbf{Fifth and finally}, we provide a decision-theoretic interpretation. We
formulate profile-guided inference as a procedure-selection problem
under uncertainty and show that the resulting procedure achieves
asymptotically vanishing regret. Under the same unique-margin and profile--loss compatibility conditions,
learning the dependence structure incurs no first-order asymptotic loss.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Introduction Part D — Paper organization
\paragraph{Related literature.}
The paper connects four literatures that have largely developed separately.
\emph{Dependence-robust inference} provides procedure-specific solutions
conditional on a known structure---heteroskedasticity- and cluster-robust
variance estimation \citep{White1980,LiangZeger1986,Arellano1987,
CameronGelbachMiller2011,CameronMiller2015}, HAC and spatial corrections
\citep{NeweyWest1987,Andrews1991,Conley1999,Conley2008,DriscollKraay1998}, and
network-robust inference \citep{Auerbach2019,Leung2022}---whereas we take the
\emph{choice} among such procedures as the object of study. \emph{Structured
covariance estimation} studies each geometry in isolation: approximate factor
structure \citep{ChamberlainRothschild1983,BaiNg2002,Bai2003}, sparse covariance
and precision estimation \citep{BickelLevina2008,CaiLiu2011,
FriedmanHastieTibshirani2008}, and low-rank-plus-sparse decompositions
\citep{CandesLiMaWright2011,Chandrasekaran2011}; we instead treat these as
competing geometries in a common Hilbert space and characterize when the data
cannot distinguish them. The \emph{model-selection and averaging} literatures
\citep{BatesGranger1969,Hansen2007,ClaeskensHjort2008} quantify relative fit; the
geometric formulation adds a notion of distance between candidate structures
themselves, enabling the local-separation and impossibility results and
connecting to adaptation theory \citep{Lepski1991}. Finally, because the
procedure selects an inference method using the same data, the oracle and regret
analysis relates to \emph{post-selection inference} \citep{LeebPoetscher2005,
BerkBrownBujaZhangZhao2013,TibshiraniEtAl2016}, delineating when selection
consistency is asymptotically innocuous and when---near overlap---no procedure
escapes the ambiguity. It also relates to the robust-statistics tradition
\citep{Huber1981,HampelEtAl1986}, where robustness concerns distributional
departures within a given dependence model rather than the dependence structure
itself; the asymptotic theory builds on standard semiparametric and
empirical-process tools \citep{BickelKlaassenRitovWellner1993,Newey1994,
VanDerVaartWellner1996,LeCamYang2000}.

The geometric formulation is not adopted merely for mathematical
convenience; it is essential relative to direct model selection based on
cross-validation, information criteria, or prediction error. It represents
heterogeneous dependence structures---clustering, latent factors, sparse
networks---within a single parameter space, so structures of very different
functional form become directly comparable; it supplies a unified notion of
distance and ambiguity, since the same Frobenius geometry that measures fit also
measures how close two candidate structures are; and it yields projection-based
identification conditions, local impossibility results, and adaptive
inference---none of which have counterparts in generic model-selection criteria,
which quantify relative fit but are silent on when candidate structures are
intrinsically indistinguishable.

\emph{Our contribution.} Existing work assumes, estimates, selects
among, or averages over covariance structures. The present paper does
not propose another covariance estimator, robust variance formula, or
selection criterion. It proposes a statistical theory for learning which
covariance geometry should govern subsequent inference: an identification
theory for when the geometry is learnable, an impossibility theory for when it
is not, and an adaptive inference theory establishing that, whenever the
geometry is learnable, learning it costs nothing asymptotically relative to
knowing it in advance. In this sense the paper shifts the focus from
dependence-robust inference under a specified covariance model to adaptive
inference under unknown dependence.

\paragraph{Theoretical roadmap and central result.}
The theory is deliberately sequential. Theorem~\ref{thm:identification} shows the
profile is well defined at regular operators and that positive principal angles
separate geometries locally; Theorems~\ref{thm:profile_consistency}
and~\ref{thm:profile_clt} transfer covariance estimation into consistent,
asymptotically normal estimation of the full and off-diagonal profiles;
Theorems~\ref{thm:dominant_geometry_consistency} and~\ref{thm:local_ties}
characterize the positive and boundary classification regimes; and
Theorem~\ref{thm:fundamental_limit} shows tangent-space overlap creates a
first-order impossibility region. The analysis culminates in
Theorem~\ref{thm:oracle_adaptivity_asymptotic_optimality}, the paper's central
data-to-decision result: whenever the dominant off-diagonal geometry is learnable
and profile rankings are compatible with inferential loss, the profile-guided
procedure is first-order equivalent to the infeasible oracle and has vanishing
regret. Each preceding result supplies a necessary link in the chain from
covariance estimation to adaptive inference.

\paragraph{Notation guide.}
Objects are introduced in pipeline order. The population operator is
$\Gamma_0\in\mathbb H_+$, estimated by $\widehat\Gamma_T$; candidate geometries
$\mathcal S_d$, $d\in\mathfrak D$, have metric projections $P_d(\Gamma)$ and
similarity scores $S_d(\Gamma)=\|P_d(\Gamma)\|_F^2$; $\omega(\Gamma)$ is the
normalized full profile and $\omega^{\mathrm{off}}(\Gamma)$ its off-diagonal
companion. The dominant population and sample geometries are $d^\star$ and
$\widehat d$, with separation margins $\Delta_{\omega^{\mathrm{off}}}$ and
$\widehat\Delta_{\omega^{\mathrm{off}}}$; $\rho_d,\widehat\rho_d$ are projection
residuals, and $\kappa_0,\widehat\kappa$ combine separation and dictionary fit.
Finally $a_d$ is the action matched to geometry $d$, $\delta$ the data-dependent
decision rule, and $\mathcal R(\delta,\Gamma_0)$ its regret. The same symbols
carry unchanged meanings in the paper, appendix, and replication code.

The paper is organized as follows. Section~\ref{sec:geometry}
introduces the statistical experiment, defines the population
dependence operator, establishes its estimability, and develops the
covariance geometry framework. Section~\ref{sec:identification}
develops geometric separation and ambiguity results.
Sections~\ref{sec:estimation} and~\ref{sec:asymptotics} study
estimation and asymptotic theory. Section~\ref{sec:classification}
develops dependence diagnostics and classification.
Section~\ref{sec:profile_guided_inference} presents profile-guided
inference. Sections~\ref{sec:simulation} and~\ref{sec:empirical}
report simulation and empirical evidence. Technical proofs and
additional results are in the Appendix. The data-to-decision pipeline is
summarized schematically in Figure~\ref{fig:workflow} of
Section~\ref{sec:profile_guided_inference}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Cov_Learn_arxiv_v2/sections/profile_guided_inference.tex <==
\section{Profile-Guided Inference}
\label{sec:profile_guided_inference}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The dependence profile provides a low-dimensional summary of the
dependence geometry encoded in an empirical dependence operator. A
natural question is whether the estimated profile can be used to guide
econometric inference. The objective of this section is not to propose a new covariance
estimator. Rather, we show how dependence learning can be combined with
existing dependence-robust procedures in a systematic way.


\begin{framed}
\noindent\textbf{Algorithm 1: Profile-Guided Adaptive Inference}
\label{alg:profile_guided}
\begin{enumerate}[leftmargin=2.2em,itemsep=0.25em,topsep=0.4em]
\item \textbf{Estimate the dependence operator.} Construct
$\widehat\Gamma_T$ from observed disturbances or residuals and, when needed,
apply the positive-semidefinite refinement described in
Section~\ref{sec:geometry}.
\item \textbf{Project onto the covariance dictionary.} For every
$d\in\mathfrak D$, compute the exact metric projection $P_d(\widehat\Gamma_T)$
or the documented numerical approximation to it.
\item \textbf{Construct diagnostics.} Compute the full profile
$\widehat\omega$, the off-diagonal profile $\widehat\omega^{\mathrm{off}}$,
and the projection residuals $\widehat\rho_d$.
\item \textbf{Assess learnability.} Determine the estimated dominant geometry
$\widehat d$, the off-diagonal margin
$\widehat\Delta_{\omega^{\mathrm{off}}}$, and the confidence index
$\widehat\kappa$.
\item \textbf{Choose an inferential action.} Apply the decision rule
$\delta(\widehat\omega^{\mathrm{off}})$: use the geometry-matched procedure
when the evidence is sufficiently separated, and use a hybrid or
multi-procedure report when the profile is ambiguous or the dictionary fit is
poor.
\end{enumerate}
\noindent\emph{Output:} the estimated dependence profile, projection-residual
diagnostics, confidence index, and recommended inference procedure.
\end{framed}


The complete procedure is the single mapping
$\widehat\Gamma_T\to(\widehat\omega,\widehat\omega^{\mathrm{off}},\widehat\rho)
\to(\widehat d,\widehat\Delta_{\omega^{\mathrm{off}}},\widehat\kappa)
\to\delta(\widehat\omega^{\mathrm{off}})\to\widehat{\mathcal P}$, where
$\widehat{\mathcal P}$ is the selected, hybrid, or multi-procedure report;
Figure~\ref{fig:workflow} displays it together with the three decision branches.

\begin{figure}[!t]
\centering
\begin{tikzpicture}[
  font=\footnotesize,
  >={Stealth[length=2mm]},
  x=1cm,y=1cm,
  proc/.style={rectangle, rounded corners=2pt, draw=black!75, fill=black!5,
               align=center, minimum height=9mm, inner sep=3pt, text width=29mm},
  hubn/.style={rectangle, rounded corners=2pt, draw=black!75, fill=black!5,
               align=center, minimum height=9mm, inner sep=3pt, text width=40mm},
  act/.style={rectangle, rounded corners=2pt, draw=black!80, fill=black!10,
              align=center, minimum height=13mm, inner sep=3pt, text width=35mm},
  arr/.style={->, draw=black!75, thick},
  lbl/.style={font=\scriptsize\itshape, fill=white, inner sep=1.5pt}
]
\node[proc] (data) at (0,6.2)  {\textbf{1.} Panel / residuals\\ $\{\widehat u_t\}_{t=1}^T$};
\node[proc] (op)   at (3.9,6.2){\textbf{2.} Estimate operator\\ $\widehat\Gamma_T=\tfrac1T\sum_t\widehat u_t\widehat u_t'$};
\node[proc] (proj) at (7.8,6.2){\textbf{3.} Project onto\\ dictionary $P_d(\widehat\Gamma_T)$};
\node[proc] (prof) at (11.7,6.2){\textbf{4.} Profiles \& residuals\\ $\widehat\omega,\widehat\omega^{\mathrm{off}},\widehat\rho_d$};
\draw[arr] (data) -- (op);
\draw[arr] (op) -- (proj);
\draw[arr] (proj) -- (prof);
\node[hubn] (learn) at (5.85,3.9) {\textbf{5.} Assess learnability:\\ $\widehat d,\ \widehat\Delta_{\omega^{\mathrm{off}}},\ \widehat\kappa=(1-\widehat\rho_{\min})\widehat\Delta_{\omega^{\mathrm{off}}}$};
\draw[arr] (prof.south) |- (learn.east);
\node[act] (matched)  at (0,1.4)  {\textbf{Matched procedure} $a_{\widehat d}$\\[1pt] \emph{oracle-equivalent}};
\node[act] (hybrid)   at (5.85,1.4){\textbf{Hybrid / multiple}\\[1pt] report several procedures};
\node[act] (caution)  at (11.7,1.4){\textbf{Caution}\\[1pt] expand dictionary; avoid geometry-specific SE};
\draw[arr] (learn.south) -- ($(learn.south)+(0,-0.55)$) -| (matched.north)
      node[lbl,pos=0.25,above]{large margin, small $\widehat\rho_{\min}$};
\draw[arr] (learn.south) -- (hybrid.north)
      node[lbl,pos=0.55]{near tie, adequate fit};
\draw[arr] (learn.south) -- ($(learn.south)+(0,-0.55)$) -| (caution.north)
      node[lbl,pos=0.25,above]{large $\widehat\rho_{\min}$};
\end{tikzpicture}
\caption{\textbf{Profile-guided adaptive inference workflow.} Steps 1--4 form the
descriptive pipeline from data to diagnostics; Step 5 summarizes learnability;
the three branches give the prescriptive action---the geometry-matched procedure
when one geometry is clearly separated and fits well (oracle-equivalent by
Theorem~\ref{thm:oracle_adaptivity_asymptotic_optimality}), a hybrid or
multi-procedure report near a tie, and a caution when the dictionary fits poorly.}
\label{fig:workflow}
\end{figure}

Algorithm~1 separates the descriptive learning problem from the prescriptive
decision problem. Steps 1--4 summarize what the data say about the covariance
dictionary; Step 5 maps that evidence into an inferential action. The oracle
result below evaluates the statistical cost of this final mapping.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Profile-Guided Procedure Recommendation}
\label{subsec:procedure_recommendation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let $\widehat d$ denote the estimated dominant geometry
of~\eqref{eq:classification_rule}. The mapping to procedures is direct: when
$\widehat\omega_C^{\mathrm{off}}$ dominates, cluster-robust procedures are the
natural benchmark; when $\widehat\omega_F^{\mathrm{off}}$ dominates,
factor-robust or common-shock-adjusted procedures; and when
$\widehat\omega_S^{\mathrm{off}}$ dominates, sparse, network, spatial, or
local-dependence robust procedures. The recommendation is evidence-based rather
than deterministic---it summarizes which geometry is most consistent with the
operator, not that one procedure is universally correct. When several scores are
substantial the data support multiple mechanisms and reporting several procedures
is preferable, and when the projection residuals indicate poor fit the entire
dictionary should be viewed with caution.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Why Learn the Geometry?}
\label{subsec:why_learn_geometry}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A natural alternative is a single broadly robust procedure---multiway
clustering, HAC inference, or a general sandwich estimator. Dependence learning
remains useful for three reasons. First, broad robustness is not costless:
procedures valid under large classes of dependence may be conservative or poorly
sized when the realized geometry differs from the structure for which they are
best suited. Second, such procedures still require the researcher to specify a
dependence class---clustering dimensions, a spatial metric, a bandwidth, or a
network---which are themselves assumptions about dependence. Third,
Theorem~\ref{thm:oracle_adaptivity_asymptotic_optimality} shows profile-guided
selection is asymptotically equivalent to an infeasible oracle that knows the
dominant geometry. Dependence learning thus provides a data-driven way to choose
among geometry-specific procedures while retaining oracle-equivalent first-order
behavior.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Procedure Confidence Index}
\label{subsec:procedure_confidence}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The reliability of a profile-based recommendation depends on two considerations:
the dominant geometry should be well separated from the competitors, and the
dictionary should approximate the operator well. Combining the estimated
separation margin
$\widehat\Delta_{\omega^{\mathrm{off}}}=\max_{d}\widehat\omega_d^{\mathrm{off}}
-\max_{d\neq\widehat d}\widehat\omega_d^{\mathrm{off}}$ with the minimum
projection residual $\widehat\rho_{\min}=\min_d\widehat\rho_d$ yields the
\emph{procedure confidence index}
\[
\widehat\kappa
=
\bigl(1-\widehat\rho_{\min}\bigr)\widehat\Delta_{\omega^{\mathrm{off}}}.
\]
Large $\widehat\kappa$ indicates that one geometry is clearly dominant
\emph{and} the dictionary fits well; small values indicate weak separation, poor
fit, or both. Its population counterpart is
$\kappa_0=(1-\rho_{\min,0})\Delta_{\omega^{\mathrm{off}},0}$, with
$\rho_{\min,0}=\min_d\rho_d$,
$\Delta_{\omega^{\mathrm{off}},0}=\max_d\omega_d^{\mathrm{off}}
-\max_{d\neq d^\star}\omega_d^{\mathrm{off}}$, and
$d^\star=\arg\max_d\omega_d^{\mathrm{off}}$.

\begin{proposition}[Consistency of the Procedure Confidence Index]
\label{prop:kappa_consistency}

Suppose the conditions of
Theorem~\ref{thm:profile_consistency} and
Assumption~\ref{ass:unique_dominant_geometry} hold, so that the dominant
geometry $d^\star$ entering $\kappa_0$ is uniquely defined. Then

\[
\widehat\kappa
\overset{p}{\longrightarrow}
\kappa_0.
\]

%
%where
%
%\[
%\kappa_0
%=
%\bigl(
%1-\rho_{\min,0}
%\bigr)
%\Delta_{\omega^{\mathrm{off}},0},
%\]
%
%\[
%\rho_{\min,0}
%=
%\min_{d\in\mathfrak D}
%\rho_d,
%\]
%
%and
%
%\[
%\Delta_{\omega^{\mathrm{off}},0}
%=
%\max_{d\in\mathfrak D}
%\omega_d
%-
%\max_{d\neq d^\star}
%\omega_d,
%\]
%
%with
%
%\[
%d^\star
%=
%\arg\max_{d\in\mathfrak D}
%\omega_d^{\mathrm{off}}.
%\]
\end{proposition}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Profile-Guided Variance Estimation}
\label{subsec:profile_guided_variance}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Suppose a scalar parameter \(\theta_0\) is estimated by \(\widehat\theta_T\).
For each geometry \(d\in\mathfrak D\), let \(\widehat V_d\) be a measurable
variance estimator and let \(\tau_{T,d}\to\infty\) be a deterministic
normalization such that
\[
\tau_{T,d}^{2}Var(\widehat\theta_T)\longrightarrow V_d,
\qquad 0<V_d<\infty.
\]
Let
\[
d^\star
=
\arg\max_{d\in\mathfrak D}
\omega_d^{\mathrm{off}}
\]
denote the dominant population dependence geometry. Define 
\[
\widehat d
=
\arg\max_{d\in\mathfrak D}\widehat\omega_d^{\mathrm{off}},
\qquad
\widehat V^{*}
=
\widehat V_{\widehat d},
\]
where ties in the argmax are broken by a fixed deterministic rule. Thus, inference is based on the variance estimator associated with the
estimated dominant dependence geometry. 

\begin{proposition}[Consistency of the Profile-Guided Variance Estimator]
\label{prop:vcov_consistency}
Let
\(
\widehat V_d
\)
denote a geometry-specific variance estimator for
\(
d\in\mathfrak D
\).
Suppose the conditions of
Theorem~\ref{thm:dominant_geometry_consistency}
hold and

\[
\widehat V_{d^\star}
\overset{p}{\longrightarrow}
V_{d^\star}.
\]
Then
\[
\widehat V^{*}
\overset{p}{\longrightarrow}
V_{d^\star}.
\]
\end{proposition}


Proposition~\ref{prop:vcov_consistency} shows that profile-guided
selection preserves consistency whenever the dominant geometry is correctly
classified. It separates the two sources of validity: geometry-specific variance
estimation supplies validity conditional on the correct geometry, while
dependence learning supplies the probability of selecting it. No new variance
formula is required.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Decision-Theoretic Formulation}
\label{subsec:decision}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The dependence profile is not itself the inferential target. It is a
sufficient low-dimensional summary for selecting among a finite dictionary
of inference procedures: operators with the same profile call for the same
procedure, so the profile retains exactly the selection-relevant
information. The decision-theoretic analysis below concerns this
procedure-selection problem, not covariance estimation per se.

The profile-guided procedure admits a natural decision-theoretic
interpretation in the sense of \citet{Wald1950}: the objective is not to estimate
the dependence structure for its own sake, but to learn enough about the
dependence geometry to select an appropriate inference procedure. Let
$\mathfrak D$ be the finite dictionary ($\mathfrak D=\{C,F,S\}$ in the baseline)
and let $L(a,\Gamma_0)$ be the loss from action $a\in\mathcal A$ when the
population operator is $\Gamma_0$. The loss may measure size distortion, coverage
error, expected interval length subject to coverage, power loss, or a weighted
combination; for example,
$L(a,\Gamma_0)=\lambda_1|P_{\Gamma_0}\{0\notin CI_a\}-\alpha|
+\lambda_2 E_{\Gamma_0}[\ell(CI_a)]$, with $CI_a$ the interval produced by $a$,
$\ell(CI_a)$ its length, and $\lambda_1,\lambda_2\ge0$ weights. The oracle rule
$\delta^\star:\Gamma\mapsto\arg\min_{a\in\mathcal A}L(a,\Gamma)$ is evaluated at
$\Gamma_0$.

\begin{assumption}[Oracle Action]
\label{ass:oracle_action}
\emph{(Profile--loss compatibility.)} The loss function and the action
set are such that the oracle rule selects the procedure associated with
the dominant dependence geometry:
$\delta^\star(\Gamma_0)=a_{d^\star}$.
\end{assumption}

\noindent
Assumption~\ref{ass:oracle_action} is a genuine restriction, not a definition:
$d^\star$ is defined by the largest similarity score---a \emph{descriptive}
ranking of fit---whereas the oracle minimizes an \emph{inferential} loss, and the
two orderings need not coincide, so the regret bound of
Theorem~\ref{thm:oracle_adaptivity_asymptotic_optimality} is conditional on their
alignment. It holds in two leading cases. \emph{(a) Size control under correct
specification:} if $a_d$ is consistent when $\Gamma_0\in\mathcal S_d$, the loss is
absolute asymptotic size distortion, and $\Gamma_0\in\mathcal S_{d^\star}$ exactly,
then $\rho_{d^\star}=0$, $d^\star$ uniquely maximizes the score, and $a_{d^\star}$
alone has zero distortion. \emph{(b) Frobenius risk:} if
$L(a_d,\Gamma_0)=\|\Gamma_0-P_d(\Gamma_0)\|_F^2$, then
by~\eqref{eq:score_residual_duality} minimizing loss is equivalent to maximizing
the score. Compatibility can also fail---if two geometries fit almost equally
well but one yields a far more variable variance estimator, a risk-based oracle
may prefer the worse-fitting but more stable procedure---so it is exactly the
statement that the loss ranks procedures the way projection distance ranks
geometries. In practice $\Gamma_0$ is unknown, and the profile-guided rule uses
the estimated profile $\widehat\omega$.

The profile-guided action is
defined as
\[
        \widehat a
        =
        \delta(\widehat\omega),
\]
where $\delta:\Delta^{|\mathfrak D|-1}\to\mathcal A$ is a decision rule
mapping dependence profiles into inference actions. A simple rule is
\[
        \delta(\widehat\omega)
        =
        a_{\widehat d},
\]
where $\widehat d$ is the estimated dominant geometry. A more conservative rule uses the separation margin
\[
        \widehat\Delta_{\omega^{\mathrm{off}}}
        =
        \widehat\omega_{\widehat d}^{\mathrm{off}}
        -
        \max_{d\neq \widehat d}\widehat\omega_d^{\mathrm{off}}
\]
and sets
\[
        \delta(\widehat\omega)
        =
        \begin{cases}
        a_{\widehat d},
        & \text{if } \widehat\Delta_{\omega^{\mathrm{off}}}>\gamma_T,\\
        a_H,
        & \text{if } \widehat\Delta_{\omega^{\mathrm{off}}}\leq \gamma_T,
        \end{cases}
\]
where $\gamma_T\downarrow 0$ is a tolerance sequence. The hybrid action
$a_H$ is intended for ambiguous regions in which no single dependence
geometry is clearly dominant.

%------------------------------------------------------------
% Risk
%------------------------------------------------------------

The risk of a decision rule $\delta$ is

\[
R(\delta,\Gamma_0)
=
E_{\Gamma_0}
\left[
L(\delta(\widehat\omega),\Gamma_0)
\right].
\]
%------------------------------------------------------------
% Regret
%------------------------------------------------------------
The regret of the profile-guided decision rule is
\[
\mathcal R(\delta,\Gamma_0)
=
E_{\Gamma_0}
\!\left[
L(\delta(\widehat\omega),\Gamma_0)
-
L(\delta^\star(\Gamma_0),\Gamma_0)
\right].
\]
Unlike estimation error, which evaluates the accuracy of an estimator,
regret evaluates the inferential cost of using a data-driven decision
rule instead of the infeasible oracle. It therefore provides a natural
decision-theoretic measure of the price of learning the dependence
structure before selecting an inference procedure.

The goal of profile-guided inference is to construct a feasible
decision rule $\delta$ whose regret converges to zero. This formalizes
the idea that learning the dependence structure before choosing an
inference procedure should not impose any first-order asymptotic loss
relative to the infeasible oracle.

It is important to be precise about \emph{what} the procedure adapts to. The
adaptivity here is not adaptivity of a covariance \emph{estimator}: the
coefficient estimator $\widehat\theta_T$ and the geometry-specific variance
estimators $\widehat V_d$ are held fixed and are not being improved. What is
learned, and what the rule adapts to, is the \emph{dependence geometry itself}---
the off-diagonal geometry $\widehat d$ that indexes which robust procedure is
appropriate. The oracle in Theorem~\ref{thm:oracle_adaptivity_asymptotic_optimality}
is the infeasible rule that \emph{knows the dominant off-diagonal geometry}
$d^\star$ and applies its matched procedure; the theorem states that using the
\emph{learned} geometry $\widehat d$ in its place costs nothing to first order.
Adaptation is therefore over the discrete set of candidate geometries, driven by
the off-diagonal dependence profile, not over a continuum of covariance
estimators.

 Let
\(
\widehat V_d
\)
be a variance estimator satisfying

\[
\widehat V_d
\overset{p}{\longrightarrow}
V_d,
\qquad
d\in\mathfrak D.
\] 
Let
\[
T_T^{*}
=
\frac{\tau_{T,\widehat {d}}\,(\widehat\theta_T-\theta_0)}
{\sqrt{\widehat V^{*}}}
\]
and
\[
T_T^{oracle}
=
\frac{\tau_{T,{d}^\star}\,(\widehat\theta_T-\theta_0)}
{\sqrt{\widehat V_{d^\star}}}.
\]

The theorem below concerns the pure profile-guided rule
$\delta(\widehat\omega)=a_{\widehat d}$. The hybrid rule is discussed as a
conservative alternative in ambiguous regions; its regret properties
require additional conditions and are not covered by the theorem.

We present the result as a corollary-strength consequence of
classification consistency rather than as a deep oracle theorem. Once
$P_{\Gamma_0}(\widehat d=d^\star)\to1$, the selected procedure coincides
with the oracle with probability tending to one and pointwise equivalence
follows almost immediately; the substantive content of the theory lies in
the identification and impossibility results, which delimit \emph{when}
classification consistency is available at all. The result is pointwise:
it is not a uniform oracle inequality, carries no regret rate, and is
silent in the near-tie region of Theorem~\ref{thm:local_ties}, where
classification consistency fails by construction. A uniform oracle
inequality or local-margin regret rate --- in particular for the hybrid
rule near ties --- would be a genuine strengthening and is left open.

\begin{theorem}[Main Theorem: Oracle Adaptivity and Decision-Theoretic Optimality]
\label{thm:oracle_adaptivity_asymptotic_optimality}
Suppose the assumptions of Theorem~\ref{thm:dominant_geometry_consistency}
hold. For part (iii), assume additionally
Assumption~\ref{ass:oracle_action} and that the loss is bounded. Then
\begin{enumerate}

\item[(i)]
The profile-guided variance estimator is asymptotically equivalent
to the infeasible oracle estimator,

\[
\widehat {V}^{*}
-
\widehat V_{d^\star}
=
o_p(1).
\]


\item[(ii)] If, in addition, the oracle statistic satisfies

\[
T_T^{oracle}
\Rightarrow
N(0,1),
\]
then

\[
T_T^{*}
-
T_T^{oracle}
=
o_p(1).
\]

Consequently,

\[
T^{*}_{T}
\Rightarrow N(0,1),
\]
whenever the oracle statistic is asymptotically standard normal. Consequently, profile-guided inference and oracle inference have the same first-order asymptotic distribution.

\item[(iii)] Assume further that the loss function satisfies
\[
|L(a,\Gamma_0)|
\le M
\]
uniformly over $a\in\mathcal A$.  The regret of the profile-guided rule satisfies
\[
        \mathcal R(\delta,\Gamma_0)       
        \to 0 .
\]

Moreover,

\[
\mathcal R(\delta,\Gamma_0)
\le
2M
P_{\Gamma_0}(\widehat d\neq d^\star)\leq
        2M
        P_{\Gamma_0}
        \left(
        \max_{d\in\mathfrak D}
        |\widehat\omega_d^{\mathrm{off}}-\omega_{d,0}^{\mathrm{off}}|
        \ge
        \frac{\Delta_{\omega^{\mathrm{off}}}}{2}
        \right),
\]

so the rate at which regret vanishes is governed by the probability of
incorrect dependence classification.

\end{enumerate}

\end{theorem}
Theorem~\ref{thm:oracle_adaptivity_asymptotic_optimality} is the central data-to-decision result of the paper and establishes the positive side of the theory.
When covariance geometries are sufficiently separated,
dependence learning consistently identifies the dominant geometry and
achieves oracle-equivalent inference with asymptotically vanishing
regret. Conversely, when the separation margin becomes small,
the oracle action itself becomes unstable because competing geometries
are locally indistinguishable. In this regime, hybrid or conservative
procedures provide a natural alternative, linking the present
decision-theoretic analysis with the impossibility result of
Section~\ref{sec:identification}.

The oracle is a benchmark for the value of learning, not an estimator available
to the researcher: at fixed separated data-generating processes, estimating the
dominant geometry has no first-order inferential cost relative to knowing it in
advance. The deliberately pointwise scope also clarifies why ambiguity
diagnostics and hybrid actions remain essential near ties.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Computation and Profile-Weighted Inference}
\label{subsec:computational_complexity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
For fixed $N$ the entire pipeline is inexpensive: constructing
$\widehat\Gamma_T$ is $O(TN^2)$ and the dominant projection cost is a dense
$O(N^3)$ eigendecomposition, with normalization, margins, residuals, and
$\widehat\kappa$ negligible by comparison. A profile-weighted alternative that
combines geometry-specific variance estimators through the estimated profile,
$\widehat V^{\mathrm{avg}}=\sum_{d}\widehat\omega_d^{\mathrm{off}}\widehat V_d$,
is also available. Computational details, scalable extensions for large $N$, and
the profile-weighted estimator are developed in Online Appendix~B.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Cov_Learn_arxiv_v2/sections/simulation_short.tex <==

\section{Simulation Evidence}
\label{sec:simulation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

This section summarizes Monte Carlo evidence on three questions: whether the
estimated profile recovers the dominant geometry, how classification behaves
under hybrid and near-tie dependence, and whether profile-guided inference
tracks the infeasible oracle that knows the dominant geometry in advance. Data-
generating processes, calibrations, projection algorithms, and additional
robustness exercises are in the Online Appendix. The baseline designs include
pure cluster, pure factor, sparse network, cluster--factor, cluster--sparse,
factor--sparse, all-three hybrid, and two-way cluster dependence.

\subsection{Dependence Learning}
\label{subsec:simulation_learning}

Table~\ref{tab:simulation_profiles} reports, for each design, the population
\emph{full dependence profile} $\boldsymbol\omega$, the population
\emph{off-diagonal dependence profile} $\boldsymbol\omega^{\mathrm{off}}$, the
population procedure confidence index $\kappa_0$, the Monte Carlo means of both
estimated profiles, and the root mean squared error of each. The off-diagonal
profile---the object that drives classification---recovers the dominant geometry
sharply in every design (e.g.\ $\omega^{\mathrm{off}}_F=0.829$ under Factor,
$\omega^{\mathrm{off}}_S=0.936$ under Sparse), whereas the full profile is pulled
toward uniformity by the common diagonal and separates the geometries far less
(cf.\ Section~\ref{sec:estimation}). The confidence index $\kappa_0$ is largest
exactly where one off-diagonal geometry is clearly separated and fits well
($\kappa_0=0.90$ under Sparse, $0.69$ under Factor) and smallest under
near-uniform or hybrid dependence. The estimation columns also make a
finite-sample point visible: with $T<N$ the sample operator is noisy, so both
estimated profiles are attenuated toward uniformity under the cluster and sparse
designs, and this is precisely what the two RMSE columns quantify. Crucially, this
attenuation shrinks the \emph{magnitudes} of the off-diagonal weights but
preserves their \emph{ordering}: the dominant geometry retains the largest
estimated off-diagonal score in each design (e.g.\ under Sparse, the estimated
sparse weight $0.477$ still exceeds the factor and cluster weights), so the
argmax classification rule remains reliable even where the profile magnitudes are
biased---a point confirmed directly by the calibration evidence in
Figure~\ref{fig:kappa_calibration}.

\begin{table}[!ht]
\centering
\caption{Estimated Dependence Profiles}
\label{tab:simulation_profiles}
\resizebox{\textwidth}{!}{%
\inputIfExists{results/tables/table_simulation_profiles.tex}%
}
\begin{minipage}{0.92\textwidth}
\footnotesize
\emph{Notes:} Columns $\omega_C,\omega_F,\omega_S$ report the population
\emph{full} dependence profile $\boldsymbol\omega$ (relative similarity to the
cluster, factor, and sparse geometries); columns
$\omega_C^{\mathrm{off}},\omega_F^{\mathrm{off}},\omega_S^{\mathrm{off}}$ report
the population \emph{off-diagonal} dependence profile
$\boldsymbol\omega^{\mathrm{off}}$; and $\kappa_0$ is the population procedure
confidence index. Columns $\widehat\omega_\bullet$ and
$\widehat\omega_\bullet^{\mathrm{off}}$ are the Monte Carlo means of the
corresponding estimated profiles over $B$ replications. The last two columns
report two distinct root mean squared errors:
$\mathrm{RMSE}(\widehat{\boldsymbol\omega})$ is the Monte Carlo root mean squared
Euclidean error of the estimated \emph{full}-profile vector, and
$\mathrm{RMSE}(\widehat{\boldsymbol\omega}^{\mathrm{off}})$ is the corresponding
error for the \emph{off-diagonal}-profile vector; for
$q\in\{\mathrm{full},\mathrm{off}\}$,
\[
\mathrm{RMSE}(\widehat{\boldsymbol\omega}^{q})
=\Bigl[B^{-1}\sum_{b=1}^{B}
\bigl\|\widehat{\boldsymbol\omega}^{q,(b)}-\boldsymbol\omega^{q}\bigr\|_2^2
\Bigr]^{1/2},
\qquad
\widehat{\boldsymbol\omega}^{\mathrm{off},(b)}
=\bigl(\widehat\omega_C^{\mathrm{off},(b)},
\widehat\omega_F^{\mathrm{off},(b)},
\widehat\omega_S^{\mathrm{off},(b)}\bigr)'.
\]
Similarity weights measure relative geometric proximity and are not additive
variance shares. The data-generating processes, calibration, and number of
replications $B$ are described in Online Appendix~E.
\end{minipage}
\end{table}

Figure~\ref{fig:hybrid_profiles} shows the average estimated off-diagonal profile
along a cluster--factor hybrid path. The profile changes smoothly as the
relative strength of factor dependence increases, illustrating that the
method summarizes hybrid dependence rather than forcing a binary
classification.

\begin{figure}[!ht]
\centering
\includegraphicsIfExists[width=.72\textwidth]{results/figures/figure_hybrid_profiles.pdf}
\caption{Dependence Profiles along a Cluster--Factor Hybrid Path}
\label{fig:hybrid_profiles}
\begin{minipage}{0.86\textwidth}
\footnotesize
\emph{Notes:} The figure plots average estimated off-diagonal similarity weights along
a path moving from cluster-dominant to factor-dominant dependence.
\end{minipage}
\end{figure}

\subsection{Classification and Ambiguity}
\label{subsec:simulation_classification}

The classification theory predicts that dominant-geometry classification
is reliable when the separation margin is large and remains probabilistic
under local near-ties. Table~\ref{tab:near_ties} reports classification
frequencies for local cluster--factor alternatives, and
Figure~\ref{fig:classification_margin} plots the relationship between
classification error and the population separation margin.

\begin{table}[!ht]
\centering
\caption{Near-Ties and Ambiguous Dependence}
\label{tab:near_ties}
\inputIfExists{results/tables/table_near_ties.tex}
\begin{minipage}{0.88\textwidth}
\footnotesize
\emph{Notes:} The table reports Monte Carlo classification frequencies
under local cluster--factor alternatives. Near-ties generate
nondegenerate classification probabilities, as predicted by the local
alternatives theory.
\end{minipage}
\end{table}

\begin{figure}[!ht]
\centering
\includegraphicsIfExists[width=.72\textwidth]{results/figures/figure_classification_margin.pdf}
\caption{Classification Error and Separation Margin}
\label{fig:classification_margin}
\begin{minipage}{0.86\textwidth}
\footnotesize
\emph{Notes:} The figure plots Monte Carlo misclassification frequency
against the population separation margin. Larger margins are associated
with lower classification error.
\end{minipage}
\end{figure}

A more demanding test is whether the procedure confidence index $\kappa_0$ is
\emph{calibrated}: does a larger $\kappa_0$ actually predict a higher probability
of recovering the dominant off-diagonal geometry? Figure~\ref{fig:kappa_calibration}
answers this along a cluster--factor path on which $\kappa_0$ sweeps from near
zero (at the crossover, where the two off-diagonal geometries tie and
Theorem~\ref{thm:fundamental_limit} predicts fundamental ambiguity) up to well-
separated values. The empirical classification probability
$\Pr(\widehat d = d^\star)$ tracks $\kappa_0$ closely: it collapses toward chance
in the near-tie region where $\kappa_0\approx0$ and rises to one once
$\kappa_0$ is bounded away from zero. The confidence index is therefore not
merely a diagnostic label but a calibrated predictor of classification
reliability---which is what licenses its use in the profile-guided decision rule.

\begin{figure}[!ht]
\centering
\includegraphicsIfExists[width=.72\textwidth]{results/figures/figure_kappa_calibration.pdf}
\caption{Calibration of the Procedure Confidence Index}
\label{fig:kappa_calibration}
\begin{minipage}{0.86\textwidth}
\footnotesize
\emph{Notes:} Monte Carlo probability of correctly identifying the dominant
off-diagonal geometry, $\Pr(\widehat d=d^\star)$, plotted against the population
procedure confidence index $\kappa_0$ along a cluster--factor mixing path. Each
point is a design on the path; vertical bars are Monte Carlo standard errors.
Accuracy falls to near chance at the near-tie point ($\kappa_0\approx0$), where
the off-diagonal tangent spaces overlap, and rises to one as $\kappa_0$
increases, showing that $\kappa_0$ is a calibrated predictor of classification
reliability.
\end{minipage}
\end{figure}

\subsection{Oracle-Equivalent Inference}
\label{subsec:simulation_oracle}

The main econometric implication of Section~\ref{sec:profile_guided_inference}
is that profile-guided inference should be asymptotically equivalent to
an infeasible oracle procedure. Table~\ref{tab:oracle_equivalence}
reports finite-sample coverage probabilities for the oracle procedure,
the profile-guided procedure, and a deliberately misspecified procedure.

\begin{table}[!ht]
\centering
\caption{Oracle Equivalence of Profile-Guided Inference}
\label{tab:oracle_equivalence}
\inputIfExists{results/tables/table_oracle_equivalence.tex}
\begin{minipage}{0.88\textwidth}
\footnotesize
\emph{Notes:} The table reports empirical coverage probabilities for
nominal 95\% confidence intervals. The oracle procedure uses the
variance estimator associated with the true dominant covariance geometry.
The profile-guided procedure uses the estimated dominant geometry. The
``Wrong Procedure'' column reports a deliberately misspecified benchmark.
\end{minipage}
\end{table}

The profile-guided procedure is nearly indistinguishable from the oracle across
the benchmark designs, while the misspecified procedure can exhibit severe
undercoverage. These results provide finite-sample support for
Theorem~\ref{thm:oracle_adaptivity_asymptotic_optimality} and the paper's main
practical message: learning the dependence profile can guide the choice of robust
inference procedure in a way that tracks the infeasible oracle benchmark.

\begin{figure}[!ht]
\centering
\includegraphicsIfExists[width=.72\textwidth]{results/figures/figure_oracle_tracking.pdf}
\caption{Oracle Tracking along a Cluster--Factor Dominance Sweep}
\label{fig:oracle_tracking}
\begin{minipage}{0.86\textwidth}
\footnotesize
\emph{Notes:} The figure compares rejection rates for fixed procedures,
the profile-guided procedure, and the infeasible oracle along a
cluster--factor dominance sweep. The profile-guided and oracle procedures
closely coincide when classification is reliable.
\end{minipage}
\end{figure}


==> Figures/del/dependence_learning_framework_v4_tikzonly_minimal.tex <==
% TikZ-only file. Include inside a figure environment with:
% \resizebox{\textwidth}{!}{\input{Figures/dependence_learning_framework_v3_tikzonly}}
% Required in main preamble:
% \usepackage{tikz}
% \usetikzlibrary{arrows,positioning,calc}
% This Version 4 preserves Version 3 layout and only increases Part B vertical spacing slightly.

\begin{tikzpicture}[
  >=stealth,
  font=\footnotesize,
  arr/.style={->, line width=0.6pt, black!80},
  panel/.style={draw=black!35, rounded corners=4pt, line width=0.55pt, fill=black!1},
  title/.style={font=\bfseries\footnotesize, text=white, fill=blue!70!black, draw=blue!70!black, rounded corners=3pt, inner xsep=6pt, inner ysep=3pt, align=center},
  flow/.style={draw=blue!65!black, fill=blue!5, rounded corners=3pt, align=center, text width=3.65cm, minimum height=0.72cm, inner sep=3pt},
  profile/.style={draw=green!45!black, fill=green!6, rounded corners=3pt, align=center, text width=3.65cm, minimum height=0.72cm, inner sep=3pt},
  diag/.style={draw=orange!75!black, fill=orange!8, rounded corners=3pt, align=center, text width=2.25cm, minimum height=0.85cm, inner sep=3pt},
  learn/.style={draw=purple!60!black, fill=purple!6, rounded corners=3pt, align=center, text width=2.25cm, minimum height=0.85cm, inner sep=3pt},
  decision/.style={draw=orange!80!black, fill=orange!9, rounded corners=3pt, align=center, text width=3.65cm, minimum height=0.72cm, inner sep=3pt},
  action/.style={draw=red!65!black, fill=red!6, rounded corners=3pt, align=center, text width=3.65cm, minimum height=0.72cm, inner sep=3pt},
  greenbox/.style={draw=green!45!black, fill=green!5, rounded corners=3pt, align=center, text width=2.75cm, minimum height=0.78cm, inner sep=3pt},
  redbox/.style={draw=red!60!black, fill=red!5, rounded corners=3pt, align=center, text width=2.75cm, minimum height=0.78cm, inner sep=3pt}
]

\node[font=\bfseries\normalsize, align=center] at (8.0,0.25)
{Overview of the Dependence Learning Framework};

\node[panel, minimum width=7.25cm, minimum height=10.55cm, anchor=north west] (PA) at (0,-0.15) {};
\node[panel, minimum width=8.35cm, minimum height=10.55cm, anchor=north west] (PB) at (7.50,-0.15) {};
\node[title, minimum width=5.65cm, anchor=north] at (3.625,-0.35) {Part A. Data-to-Decision Pipeline};
\node[title, minimum width=6.50cm, anchor=north] at (11.675,-0.35) {Part B. Identification and Fundamental Limits};

% Part A
\node[flow] (A1) at (3.625,-1.35) {Data\\[-1pt] $\{y_{it},x_{it}\}$};
\node[flow] (A2) at (3.625,-2.55) {Empirical operator\\[-1pt] $\widehat{\Gamma}_n\in\mathcal H$};
\node[flow] (A3) at (3.625,-3.75) {Geometry projection\\[-1pt] $\{\mathcal G_1,\ldots,\mathcal G_K\}$};
\node[profile] (A4) at (3.625,-4.95) {Geometric profile\\[-1pt] $\widehat\omega=(\widehat\omega_1,\ldots,\widehat\omega_K)$};
\node[diag] (A5a) at (1.95,-6.30) {Diagnostics\\[-1pt] $\widehat r_n$};
\node[learn] (A5b) at (5.30,-6.30) {Learning\\[-1pt] $\widehat d$, ambiguity};
\node[decision] (A6) at (3.625,-7.72) {Decision rule\\[-1pt] $a=\delta(\widehat\omega,\widehat r_n)$};
\node[action] (A7) at (3.625,-8.92) {Adaptive inference\\[-1pt] $V_n=V_n(a,\widehat\omega)$};
\draw[arr] (A1) -- (A2); \draw[arr] (A2) -- (A3); \draw[arr] (A3) -- (A4);
\draw[arr] (A4.south west) -- (A5a.north); \draw[arr] (A4.south east) -- (A5b.north);
\draw[arr] (A5a.south) |- (A6.west); \draw[arr] (A5b.south) |- (A6.east); \draw[arr] (A6) -- (A7);

% Part B
\node[font=\bfseries\footnotesize, text=green!40!black, align=center] at (9.65,-1.18)
{Separated geometries\\[-1pt] \normalfont identifiable};
\node[font=\bfseries\footnotesize, text=red!65!black, align=center] at (13.65,-1.18)
{Overlapping geometries\\[-1pt] \normalfont nonidentifiable};
\draw[green!45!black, fill=green!12, line width=0.6pt] (8.65,-1.95) -- (9.25,-1.78) -- (9.72,-2.05) -- (8.98,-2.27) -- cycle;
\draw[blue!65!black, fill=blue!10, line width=0.6pt] (10.20,-2.20) -- (10.90,-2.02) -- (11.18,-1.70) -- (10.38,-1.88) -- cycle;
\draw[<->, >=stealth, black!70, line width=0.5pt] (9.80,-2.05) to[bend left=20] node[above, font=\tiny] {$\theta_{jk}>0$} (10.15,-2.05);
\draw[red!65!black, fill=red!10, line width=0.6pt] (12.20,-1.98) -- (12.98,-1.80) -- (13.25,-2.23) -- (12.42,-2.42) -- cycle;
\draw[blue!65!black, fill=blue!10, line width=0.6pt, opacity=0.75] (12.85,-2.23) -- (13.72,-2.03) -- (14.10,-2.28) -- (13.22,-2.58) -- cycle;
\node[font=\tiny] at (14.08,-2.65) {$\theta_{jk}=0$};

\node[greenbox] (B1) at (9.65,-3.45) {Identification\\[-1pt] \tiny separated tangents};
\node[greenbox] (B2) at (9.65,-4.67) {Consistent profile\\[-1pt] $\widehat\omega\overset{p}{\to}\omega$};
\node[greenbox] (B3) at (9.65,-5.89) {Dependence learning\\[-1pt] $\Pr(\widehat d=d^\star)\to1$};
\node[greenbox] (B4) at (9.65,-7.11) {Oracle inference\\[-1pt] $V_n-V_n^{oracle}=o_p(n^{-1/2})$};
\node[greenbox] (B5) at (9.65,-8.33) {Vanishing regret\\[-1pt] $\mathcal R_n=o(1)$};
\node[redbox] (C1) at (13.65,-3.45) {Fundamental limit\\[-1pt] \tiny overlapping tangents};
\node[redbox] (C2) at (13.65,-4.67) {Indistinguishability\\[-1pt] \tiny no first-order test};
\node[redbox] (C3) at (13.65,-5.89) {Ambiguous profile\\[-1pt] \tiny diffuse $\widehat\omega$};
\node[redbox] (C4) at (13.65,-7.11) {Hybrid action\\[-1pt] \tiny minimax or mixture};
\node[redbox] (C5) at (13.65,-8.33) {Positive regret\\[-1pt] \tiny unavoidable near overlap};
\draw[arr] (B1) -- (B2); \draw[arr] (B2) -- (B3); \draw[arr] (B3) -- (B4); \draw[arr] (B4) -- (B5);
\draw[arr] (C1) -- (C2); \draw[arr] (C2) -- (C3); \draw[arr] (C3) -- (C4); \draw[arr] (C4) -- (C5);

\end{tikzpicture}


==> Figures/dependence_learning_framework_v4_tikzonly_minimal.tex <==
% TikZ-only file. Include inside a figure environment with:
% \resizebox{\textwidth}{!}{\input{Figures/dependence_learning_framework_v3_tikzonly}}
% Required in main preamble:
% \usepackage{tikz}
% \usetikzlibrary{arrows,positioning,calc}
% This Version 4 preserves Version 3 layout and only increases Part B vertical spacing slightly.

\begin{tikzpicture}[
  >=stealth,
  font=\footnotesize,
  arr/.style={->, line width=0.6pt, black!80},
  panel/.style={draw=black!35, rounded corners=4pt, line width=0.55pt, fill=black!1},
  title/.style={font=\bfseries\footnotesize, text=white, fill=blue!70!black, draw=blue!70!black, rounded corners=3pt, inner xsep=6pt, inner ysep=3pt, align=center},
  flow/.style={draw=blue!65!black, fill=blue!5, rounded corners=3pt, align=center, text width=3.65cm, minimum height=0.72cm, inner sep=3pt},
  profile/.style={draw=green!45!black, fill=green!6, rounded corners=3pt, align=center, text width=3.65cm, minimum height=0.72cm, inner sep=3pt},
  diag/.style={draw=orange!75!black, fill=orange!8, rounded corners=3pt, align=center, text width=2.25cm, minimum height=0.85cm, inner sep=3pt},
  learn/.style={draw=purple!60!black, fill=purple!6, rounded corners=3pt, align=center, text width=2.25cm, minimum height=0.85cm, inner sep=3pt},
  decision/.style={draw=orange!80!black, fill=orange!9, rounded corners=3pt, align=center, text width=3.65cm, minimum height=0.72cm, inner sep=3pt},
  action/.style={draw=red!65!black, fill=red!6, rounded corners=3pt, align=center, text width=3.65cm, minimum height=0.72cm, inner sep=3pt},
  greenbox/.style={draw=green!45!black, fill=green!5, rounded corners=3pt, align=center, text width=2.75cm, minimum height=0.78cm, inner sep=3pt},
  redbox/.style={draw=red!60!black, fill=red!5, rounded corners=3pt, align=center, text width=2.75cm, minimum height=0.78cm, inner sep=3pt}
]

\node[font=\bfseries\normalsize, align=center] at (8.0,0.25)
{Overview of the Dependence Learning Framework};

\node[panel, minimum width=7.25cm, minimum height=10.55cm, anchor=north west] (PA) at (0,-0.15) {};
\node[panel, minimum width=8.35cm, minimum height=10.55cm, anchor=north west] (PB) at (7.50,-0.15) {};
\node[title, minimum width=5.65cm, anchor=north] at (3.625,-0.35) {Part A. Data-to-Decision Pipeline};
\node[title, minimum width=6.50cm, anchor=north] at (11.675,-0.35) {Part B. Identification and Fundamental Limits};

% Part A
\node[flow] (A1) at (3.625,-1.35) {Data\\[-1pt] $\{y_{it},x_{it}\}$};
\node[flow] (A2) at (3.625,-2.55) {Empirical operator\\[-1pt] $\widehat{\Gamma}_T\in\mathcal H$};
\node[flow] (A3) at (3.625,-3.75) {Geometry projection\\[-1pt] $\{\mathcal G_1,\ldots,\mathcal G_K\}$};
\node[profile] (A4) at (3.625,-4.95) {Geometric profile\\[-1pt] $\widehat\omega=(\widehat\omega_1,\ldots,\widehat\omega_K)$};
\node[diag] (A5a) at (1.95,-6.30) {Diagnostics\\[-1pt] $\widehat r_T$};
\node[learn] (A5b) at (5.30,-6.30) {Learning\\[-1pt] $\widehat d$, ambiguity};
\node[decision] (A6) at (3.625,-7.72) {Decision rule\\[-1pt] $a=\delta(\widehat\omega,\widehat r_T)$};
\node[action] (A7) at (3.625,-8.92) {Adaptive inference\\[-1pt] $V_T=V_T(a,\widehat\omega)$};
\draw[arr] (A1) -- (A2); \draw[arr] (A2) -- (A3); \draw[arr] (A3) -- (A4);
\draw[arr] (A4.south west) -- (A5a.north); \draw[arr] (A4.south east) -- (A5b.north);
\draw[arr] (A5a.south) |- (A6.west); \draw[arr] (A5b.south) |- (A6.east); \draw[arr] (A6) -- (A7);

% Part B
\node[font=\bfseries\footnotesize, text=green!40!black, align=center] at (9.65,-1.18)
{Separated geometries\\[-1pt] \normalfont identifiable};
\node[font=\bfseries\footnotesize, text=red!65!black, align=center] at (13.65,-1.18)
{Overlapping geometries\\[-1pt] \normalfont nonidentifiable};
\draw[green!45!black, fill=green!12, line width=0.6pt] (8.65,-1.95) -- (9.25,-1.78) -- (9.72,-2.05) -- (8.98,-2.27) -- cycle;
\draw[blue!65!black, fill=blue!10, line width=0.6pt] (10.20,-2.20) -- (10.90,-2.02) -- (11.18,-1.70) -- (10.38,-1.88) -- cycle;
\draw[<->, >=stealth, black!70, line width=0.5pt] (9.80,-2.05) to[bend left=20] node[above, font=\tiny] {$\theta_{jk}>0$} (10.15,-2.05);
\draw[red!65!black, fill=red!10, line width=0.6pt] (12.20,-1.98) -- (12.98,-1.80) -- (13.25,-2.23) -- (12.42,-2.42) -- cycle;
\draw[blue!65!black, fill=blue!10, line width=0.6pt, opacity=0.75] (12.85,-2.23) -- (13.72,-2.03) -- (14.10,-2.28) -- (13.22,-2.58) -- cycle;
\node[font=\tiny] at (14.08,-2.65) {$\theta_{jk}=0$};

\node[greenbox] (B1) at (9.65,-3.45) {Identification\\[-1pt] \tiny separated tangents};
\node[greenbox] (B2) at (9.65,-4.67) {Consistent profile\\[-1pt] $\widehat\omega\overset{p}{\to}\omega$};
\node[greenbox] (B3) at (9.65,-5.89) {Dependence learning\\[-1pt] $\Pr(\widehat d=d^\star)\to1$};
\node[greenbox] (B4) at (9.65,-7.11) {Oracle inference\\[-1pt] $V_T-V_T^{oracle}=o_p(T^{-1/2})$};
\node[greenbox] (B5) at (9.65,-8.33) {Vanishing regret\\[-1pt] $\mathcal R_T=o(1)$};
\node[redbox] (C1) at (13.65,-3.45) {Fundamental limit\\[-1pt] \tiny overlapping tangents};
\node[redbox] (C2) at (13.65,-4.67) {Indistinguishability\\[-1pt] \tiny no first-order test};
\node[redbox] (C3) at (13.65,-5.89) {Ambiguous profile\\[-1pt] \tiny diffuse $\widehat\omega$};
\node[redbox] (C4) at (13.65,-7.11) {Hybrid action\\[-1pt] \tiny minimax or mixture};
\node[redbox] (C5) at (13.65,-8.33) {Positive regret\\[-1pt] \tiny unavoidable near overlap};
\draw[arr] (B1) -- (B2); \draw[arr] (B2) -- (B3); \draw[arr] (B3) -- (B4); \draw[arr] (B4) -- (B5);
\draw[arr] (C1) -- (C2); \draw[arr] (C2) -- (C3); \draw[arr] (C3) -- (C4); \draw[arr] (C4) -- (C5);

\end{tikzpicture}


==> sections/dependence_learning_conceptual_figure_tikz.tex <==
% Requires in the preamble:
% \usepackage{tikz}
% \usetikzlibrary{arrows.meta,calc}
% \usepackage{graphicx}
% \usepackage{amsmath,amssymb}

\begin{figure}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tikzpicture}[
    >=Latex,
    font=\footnotesize,
    line/.style={-{Latex[length=2.2mm,width=1.3mm]}, line width=0.5pt},
    panel/.style={rectangle, rounded corners=5pt, draw=blue!65, fill=white, line width=0.8pt},
    titlebar/.style={rectangle, rounded corners=3pt, draw=blue!70!black, fill=blue!70!black,
        text=white, font=\bfseries\footnotesize, align=center, inner ysep=3pt},
    stepblue/.style={rectangle, rounded corners=3pt, draw=blue!60, fill=blue!4,
        align=center, text width=7.2cm, minimum height=0.90cm, inner xsep=5pt, inner ysep=4pt, line width=0.45pt},
    stepgreen/.style={rectangle, rounded corners=3pt, draw=green!45!black, fill=green!5,
        align=center, text width=7.35cm, minimum height=1.00cm, inner xsep=5pt, inner ysep=4pt, line width=0.45pt},
    sideorange/.style={rectangle, rounded corners=3pt, draw=orange!80!black, fill=orange!7,
        align=left, text width=4.35cm, minimum height=2.65cm, inner xsep=6pt, inner ysep=6pt, line width=0.45pt},
    sidepurple/.style={rectangle, rounded corners=3pt, draw=purple!70, fill=purple!6,
        align=left, text width=4.55cm, minimum height=2.65cm, inner xsep=6pt, inner ysep=6pt, line width=0.45pt},
    steporange/.style={rectangle, rounded corners=3pt, draw=orange!80!black, fill=orange!7,
        align=center, text width=7.35cm, minimum height=1.00cm, inner xsep=5pt, inner ysep=4pt, line width=0.45pt},
    stepred/.style={rectangle, rounded corners=3pt, draw=red!60, fill=red!5,
        align=center, text width=7.35cm, minimum height=1.15cm, inner xsep=5pt, inner ysep=4pt, line width=0.45pt},
    theorygreen/.style={rectangle, rounded corners=3pt, draw=green!45!black, fill=green!5,
        align=center, text width=4.15cm, minimum height=1.15cm, inner xsep=4pt, inner ysep=4pt, line width=0.45pt},
    theoryred/.style={rectangle, rounded corners=3pt, draw=red!55, fill=red!5,
        align=center, text width=4.15cm, minimum height=1.15cm, inner xsep=4pt, inner ysep=4pt, line width=0.45pt}
]

% =====================================================
% Part A: data-to-decision pipeline
% =====================================================
\node[panel, minimum width=10.7cm, minimum height=16.1cm, anchor=north west] (panelA) at (0,0) {};
\node[titlebar, minimum width=8.1cm, anchor=north] at ([yshift=-0.18cm]panelA.north)
{Part A. The Data-to-Decision Pipeline};
\node[font=\itshape, align=center, text width=9.8cm, anchor=north] at ([yshift=-0.90cm]panelA.north)
{From observed data to adaptive inference via dependence learning.};

\node[stepblue, anchor=north] (A1) at ([yshift=-1.80cm]panelA.north)
{\textbf{1. Observed data}\\[-1pt]$\{y_{it},x_{it}\}$};
\node[stepblue, anchor=north] (A2) at ([yshift=-3.15cm]panelA.north)
{\textbf{2. Estimate dependence operator}\\[-1pt]$\widehat{\Gamma}_T\in\mathcal H$};
\node[stepblue, anchor=north] (A3) at ([yshift=-4.50cm]panelA.north)
{\textbf{3. Project onto covariance geometries}\\[-1pt]$\{\mathcal G_1,\ldots,\mathcal G_K\}$};
\node[stepgreen, anchor=north] (A4) at ([yshift=-5.85cm]panelA.north)
{\textbf{4. Geometric dependence profile}\\[-1pt]$\omega=(\omega_1,\ldots,\omega_K)\in\Delta^{K-1}$};
\node[stepgreen, anchor=north] (A5) at ([yshift=-7.35cm]panelA.north)
{\textbf{5. Estimated profile}\\[-1pt]$\widehat{\omega}=(\widehat{\omega}_1,\ldots,\widehat{\omega}_K)$};

\node[sideorange, anchor=north west] (A6a) at ([xshift=0.45cm,yshift=-8.95cm]panelA.north west)
{\centering\textbf{6a. Projection diagnostics}\par\vspace{3pt}
$\bullet$ Dictionary projection residual $\widehat r_T$\\[3pt]
$\bullet$ Misspecification assessment\\[3pt]
$\bullet$ Absolute fit of the dictionary};

\node[sidepurple, anchor=north east] (A6b) at ([xshift=-0.45cm,yshift=-8.95cm]panelA.north east)
{\centering\textbf{6b. Dependence learning}\par\vspace{3pt}
$\bullet$ Identify dominant geometry\\[-1pt]
\hspace*{0.4cm}$\widehat d=\arg\max_k\widehat\omega_k$\\[3pt]
$\bullet$ Assess ambiguity\\[3pt]
$\bullet$ Quantify uncertainty};

\node[steporange, anchor=north] (A7) at ([yshift=-12.35cm]panelA.north)
{\textbf{7. Decision rule}\\[-1pt]
$\delta(\widehat\omega,\widehat r_T)\mapsto a\in\mathcal A$};
\node[stepred, anchor=north] (A8) at ([yshift=-13.90cm]panelA.north)
{\textbf{8. Adaptive inference action}\\[-1pt]
Implement dependence-robust procedure\\[-1pt]
$V_T=V_T(a,\widehat\omega)$};

\draw[line] (A1) -- (A2);
\draw[line] (A2) -- (A3);
\draw[line] (A3) -- (A4);
\draw[line] (A4) -- (A5);
\draw[line] (A5.south) -- ++(0,-0.36) -| (A6a.north);
\draw[line] (A5.south) -- ++(0,-0.36) -| (A6b.north);
\draw[line] (A6a.south) |- (A7.west);
\draw[line] (A6b.south) |- (A7.east);
\draw[line] (A7) -- (A8);

% =====================================================
% Part B: geometric regimes and consequences
% =====================================================
\node[panel, minimum width=10.0cm, minimum height=16.1cm, anchor=north west] (panelB) at (11.05,0) {};
\node[titlebar, minimum width=8.7cm, anchor=north] at ([yshift=-0.18cm]panelB.north)
{Part B. Geometric Regimes and Inferential Consequences};
\node[font=\itshape, align=center, text width=8.9cm, anchor=north] at ([yshift=-0.90cm]panelB.north)
{Theoretical dichotomy determined by the geometry of covariance classes.};

\node[draw=green!45!black, fill=green!3, rounded corners=4pt,
      minimum width=4.55cm, minimum height=13.95cm, anchor=north west, line width=0.55pt]
      (Bleftpanel) at ([xshift=0.45cm,yshift=-1.78cm]panelB.north west) {};
\node[draw=red!55, fill=red!3, rounded corners=4pt,
      minimum width=4.55cm, minimum height=13.95cm, anchor=north east, line width=0.55pt]
      (Brightpanel) at ([xshift=-0.45cm,yshift=-1.78cm]panelB.north east) {};

\node[font=\bfseries\color{green!40!black}, align=center, text width=4.2cm, anchor=north]
      (Bltitle) at ([yshift=-2.08cm]panelB.north west -| Bleftpanel.center)
{Separated geometries\\(identifiable regime)};
\node[font=\bfseries\color{red!60!black}, align=center, text width=4.2cm, anchor=north]
      (Brtitle) at ([yshift=-2.08cm]panelB.north east -| Brightpanel.center)
{Overlapping geometries\\(nonidentifiable regime)};

\node[theorygreen, anchor=north] (B1) at ([yshift=-3.65cm]panelB.north west -| Bleftpanel.center)
{\textbf{Identification}\\[-1pt]$\theta_{jk}>0$};
\node[theorygreen, anchor=north] (B2) at ([yshift=-5.90cm]panelB.north west -| Bleftpanel.center)
{\textbf{Consistent profile}\\[-1pt]$\widehat\omega\overset{p}{\longrightarrow}\omega$};
\node[theorygreen, anchor=north] (B3) at ([yshift=-8.15cm]panelB.north west -| Bleftpanel.center)
{\textbf{Dependence learning}\\[-1pt]$P_{\Gamma_0}(\widehat d=d^\star)\to1$};
\node[theorygreen, anchor=north] (B4) at ([yshift=-10.40cm]panelB.north west -| Bleftpanel.center)
{\textbf{Oracle adaptivity}\\[-1pt]$\sqrt T\{V_T-V_T^{\mathrm{oracle}}\}=o_p(1)$};
\node[theorygreen, anchor=north] (B5) at ([yshift=-12.65cm]panelB.north west -| Bleftpanel.center)
{\textbf{Vanishing regret}\\[-1pt]$\mathcal R_n=o(1)$};

\draw[line] (B1) -- (B2);
\draw[line] (B2) -- (B3);
\draw[line] (B3) -- (B4);
\draw[line] (B4) -- (B5);

\node[theoryred, anchor=north] (C1) at ([yshift=-3.65cm]panelB.north east -| Brightpanel.center)
{\textbf{Fundamental limit}\\[-1pt]$\theta_{jk}=0$};
\node[theoryred, anchor=north] (C2) at ([yshift=-5.90cm]panelB.north east -| Brightpanel.center)
{\textbf{Local indistinguishability}\\[-1pt]No first-order test};
\node[theoryred, anchor=north] (C3) at ([yshift=-8.15cm]panelB.north east -| Brightpanel.center)
{\textbf{Ambiguous profile}\\[-1pt]$\widehat\omega$ remains diffuse};
\node[theoryred, anchor=north] (C4) at ([yshift=-10.40cm]panelB.north east -| Brightpanel.center)
{\textbf{Hybrid / robust action}\\[-1pt]Mixture or minimax rule};
\node[theoryred, anchor=north] (C5) at ([yshift=-12.65cm]panelB.north east -| Brightpanel.center)
{\textbf{Positive regret unavoidable}\\[-1pt]No uniformly oracle rule};

\draw[line] (C1) -- (C2);
\draw[line] (C2) -- (C3);
\draw[line] (C3) -- (C4);
\draw[line] (C4) -- (C5);

% Bottom note
\node[draw=blue!55, dashed, rounded corners=3pt, align=center, text width=19.4cm,
      fill=blue!2, inner xsep=5pt, inner ysep=6pt, anchor=north]
      at (10.55,-16.55)
{Part A summarizes the data-to-decision pipeline: estimate a dependence operator, construct the geometric dependence profile $\widehat\omega$, conduct diagnostics and learning, and select an inference action. Part B summarizes the two geometric regimes that determine the possibilities and limits of dependence learning and adaptive inference.};

\end{tikzpicture}%
}
\caption{From dependence learning to adaptive inference. Part A summarizes the data-to-decision pipeline: observed data are used to estimate a dependence operator, which is projected onto candidate covariance geometries to construct the full and off-diagonal dependence profiles $(\widehat\omega,\widehat\omega^{\mathrm{off}})$. The off-diagonal profile is primary for classification, while the full profile and projection diagnostics are then mapped into an inference action through a decision rule. Part B summarizes the two geometric regimes underlying the theory. When covariance geometries are separated, the dependence profile is identifiable, dependence learning is consistent, and profile-guided inference achieves oracle equivalence with vanishing regret. When covariance geometries overlap, local indistinguishability generates intrinsic ambiguity and motivates hybrid or robust inference actions.}
\label{fig:dependence-learning-framework}
\end{figure}

